Total Error and Variability Measures for the Quarterly Workforce Indicators and LEHD Origin-Destination Employment Statistics in OnTheMap

We report results from the first comprehensive total quality evaluation of five major indicators in the U.S. Census Bureau's Longitudinal Employer-Household Dynamics (LEHD) Program Quarterly Workforce Indicators (QWI): total flow-employment, beginning-of-quarter employment, full-quarter employment, average monthly earnings of full-quarter employees, and total quarterly payroll. Beginning-of-quarter employment is also the main tabulation variable in the LEHD Origin-Destination Employment Statistics (LODES) workplace reports as displayed in OnTheMap (OTM), including OnTheMap for Emergency Management. We account for errors due to coverage; record-level non-response; edit and imputation of item missing data; and statistical disclosure limitation. The analysis reveals that the five publication variables under study are estimated very accurately for tabulations involving at least 10 jobs. Tabulations involving three to nine jobs are a transition zone, where cells may be fit for use with caution. Tabulations involving one or two jobs, which are generally suppressed on fitness-for-use criteria in the QWI and synthesized in LODES, have substantial total variability but can still be used to estimate statistics for untabulated aggregates as long as the job count in the aggregate is more than 10.

==> figures/education.tex <==
\begin{figure}
        \centering
         \subfigure[Less than High School]{%
            \label{fig:lesshs}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/less_hs.pdf}
         } \qquad%
	      \subfigure[High School]{%
            \label{fig:hs}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/hs.pdf}
         } \\ %
         \subfigure[Some College]{%
            \label{fig:somecollege}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/somecollege.pdf}
         } \qquad%
	      \subfigure[Bachelor's degree and above]{%
            \label{fig:baplus}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/college.pdf}
         } \\ %

        \caption{Impute versus Target: Education}
        \label{fig:impeducation}
\footnotesize
\begin{flushleft} {\it Notes}: Sub-figure titles correspond to the value of the education variable in the ICF. The blue bars show the distribution of education in the ICF among records that were not imputed. The red bars shows the distribution of education in the ICF among imputed records. The green bars show the distribution of education among records in the ICF that were not imputed {\em and} did not match to the ACS. The green bars do not vary across sub-figures. See Table \ref{tab:imped} for more detail.
\end{flushleft}%  
\end{figure}%

%\usepackage{subfig} %handles subfloats 


==> figures/ethnicity.tex <==
\begin{figure}
        \centering
         \subfigure[Not Hispanic]{%
            \label{fig:nonhis}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/not_hispanic.pdf}
         } \qquad%
	      \subfigure[Hispanic]{%
            \label{fig:his}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/hispanic.pdf}
         } \\ %

        \caption{Impute versus Target: Ethnicity}
        \label{fig:impethnicity}
\footnotesize
\begin{flushleft} {\it Notes}: Sub-figure titles correspond to the value of the ethnicity variable in the ICF. The blue bars show the distribution of ethnicity in the ICF among records that were not imputed. The red bars shows the distribution of ethnicity in the ICF among imputed records. The green bars show the distribution of ethnicity among records in the ICF that were not imputed {\em and} did not match to the ACS. The green bars do not vary across sub-figures. See Table \ref{tab:impeth} for more detail.

\end{flushleft}%  
\end{figure}%


==> figures/race.tex <==
\begin{figure}
        \centering
         \subfigure[White]{%
            \label{fig:white}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/white.pdf}
         } \qquad%
	      \subfigure[Black]{%
            \label{fig:black}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/black.pdf}
         } \\ %
         \subfigure[Asian]{%
            \label{fig:asian}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/asian.pdf}
         } \qquad%
	      \subfigure[Native American or Alaska Native]{%
            \label{fig:naan}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/native_american.pdf}
         } \\ %
         \subfigure[Hawaiian or Pacific Islander]{%
            \label{fig:hwpi}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/hawaiian_pi.pdf}
         } \qquad%
	      \subfigure[Two or More Races]{%
            \label{fig:twoplus}%
            \includegraphics[scale=0.25]{\MyPathtv/figures/twoormore.pdf}
         } \\ %


        \caption{Impute versus Target: Race}
        \label{fig:imprace}
\footnotesize
\begin{flushleft} {\it Notes}: Sub-figure titles correspond to the value of the race variable in the ICF. The blue bars show the distribution of race in the ICF among records that were not imputed. The red bars shows the distribution of race in the ICF among imputed records. The green bars show the distribution of race among records in the ICF that were not imputed {\em and} did not match to the ACS. The green bars do not vary across sub-figures. See Table \ref{tab:imprace} for more detail.

\end{flushleft}%  
\end{figure}%

%\usepackage{subfig} %handles subfloats 


==> tables/ame_table.tex <==
\begin{landscape}
\begin{table}[htbp]
    \resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of Average Monthly Earnings ($EarnS$) by Table and Count}
\begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 15}{c}{} \\ 

\multicolumn{ 1}{c}{Table and $EmpS$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Count} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Bounds Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
\multicolumn{15}{c}{\textbf{A: Private}} \\ 

\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Average Monthly Earnings is defined only over full-quarter jobs. It is calculated by taking the earnings for the reference quarter for full-quarter jobs and dividing by 3.  See the table on full-quarter employment for the relevent counts. Statistics are computed across all state-year-quarters within a table. The ``All" category of establishments includes private as well as state, and local government but excludes federal employment. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for beginning of quarter employment, please see their respective equations in the accompanying text:  Average Monthly Earnings \ref{eq:z3pub}, Total Variation \ref{eq:tvz}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.  
 (a) Undefined value.
\end{tablenotes}
\end{threeparttable}
}%
\label{tab:ame}
\end{table}
\end{landscape}



==> tables/ame_table_a.tex <==
Age x Gender & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad 100-999 & 0.0001 &  6  & 1,686.00  &  &  13,600.00  & 87.00\% &  & 0.0691 & 0.0691 & 0.0691 &  & 11 & 159.00 & 9.42\% \\ 
\quad +1000 & 0.9999 &  44,938  & 2,146.00  &  &  6.79  & 22.90\% &  & 0.0004 & 0.0013 & 0.0066 &  & 171 & 3.35 & 0.17\% \\ 
Race x Ethnicity & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad 3-9 & 0.0005 &  17  & 2,409.00  &  &  361,000.00  & 96.80\% &  & 0.1451 & 0.2600 & 0.6976 &  & 9 & 830.97 & 35.95\% \\ 
\quad 10-99 & 0.0351 &  1,184  & 2,106.50  &  &  71,000.00  & 95.50\% &  & 0.0605 & 0.1252 & 0.3384 &  & 9 & 368.52 & 17.31\% \\ 
\quad 100-999 & 0.1780 &  6,001  & 2,189.00  &  &  8,490.00  & 94.50\% &  & 0.0147 & 0.0425 & 0.1042 &  & 10 & 126.43 & 5.84\% \\ 
\quad +1000 & 0.7863 &  26,506  & 2,471.00  &  &  168.00  & 73.70\% &  & 0.0004 & 0.0052 & 0.0321 &  & 16 & 17.33 & 0.69\% \\ 
Gender x Education & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad +1000 & 1.0000 &  22,472  & 2,847.00  &  &  84.60  & 94.40\% &  & 0.0013 & 0.0032 & 0.0088 &  & 10 & 12.62 & 0.44\% \\ 
Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0020 &  6,177  & 0.00  &  &  2,140,000.00  & 99.30\% &  & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 2023.20 & (a) \\ 
\quad 1-2 & 0.1096 &  342,768  & 2,088.00  &  &  7,230.00  & 0.00\% &  & 0.0000 & 0.0545 & 0.2903 &  & 9999 & 108.98 & 6.98\% \\ 
\quad 3-9 & 0.0294 &  92,014  & 1,523.00  &  &  8,540.00  & 0.00\% &  & 0.0202 & 0.0655 & 0.2728 &  & 9999 & 118.44 & 8.39\% \\ 
\quad 10-99 & 0.2836 &  886,839  & 1,957.00  &  &  5,240.00  & 11.20\% &  & 0.0150 & 0.0385 & 0.1256 &  & 714 & 92.85 & 4.93\% \\ 
\quad 100-999 & 0.3749 &  1,172,234  & 2,265.00  &  &  2,020.00  & 65.80\% &  & 0.0081 & 0.0207 & 0.0551 &  & 20 & 59.57 & 2.75\% \\ 
\quad +1000 & 0.2005 &  626,901  & 2,701.00  &  &  414.00  & 70.60\% &  & 0.0026 & 0.0080 & 0.0216 &  & 18 & 27.07 & 1.07\% \\ 
Age x Gender x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0025 &  98,832  & 0.00  &  &  2,690,000.00  & 99.60\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 2268.34 & (a) \\ 
\quad 1-2 & 0.2269 &  8,953,462  & 1,297.00  &  &  9,140.00  & 0.00\% &  & 0.0000 & 0.0850 & 0.4718 &  & 9999 & 122.53 & 10.90\% \\ 
\quad 3-9 & 0.2410 &  9,509,759  & 1,479.00  &  &  17,400.00  & 66.90\% &  & 0.0280 & 0.0932 & 0.2942 &  & 20 & 174.82 & 12.35\% \\ 
\quad 10-99 & 0.3668 &  14,475,571  & 1,828.00  &  &  8,620.00  & 74.70\% &  & 0.0210 & 0.0538 & 0.1433 &  & 16 & 124.11 & 7.19\% \\ 
\quad 100-999 & 0.1372 &  5,413,281  & 2,300.00  &  &  2,280.00  & 77.30\% &  & 0.0087 & 0.0224 & 0.0545 &  & 15 & 64.01 & 3.00\% \\ 
\quad +1000 & 0.0258 &  1,017,595  & 3,109.00  &  &  578.00  & 72.90\% &  & 0.0033 & 0.0084 & 0.0204 &  & 16 & 32.14 & 1.12\% \\ 
Race x Ethnicity x Inudstry x  County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0043 &  74,124  & 0.00  &  &  6,290,000.00  & 99.90\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 3468.62 & (a) \\ 
\quad 1-2 & 0.3501 &  5,991,260  & 1,835.00  &  &  226,000.00  & 97.20\% &  & 0.0499 & 0.2686 & 0.7331 &  & 9 & 657.48 & 37.15\% \\ 
\quad 3-9 & 0.2141 &  3,664,172  & 1,942.00  &  &  126,000.00  & 93.50\% &  & 0.0563 & 0.1853 & 0.4744 &  & 10 & 487.08 & 25.42\% \\ 
\quad 10-99 & 0.2557 &  4,375,170  & 2,082.00  &  &  24,500.00  & 86.80\% &  & 0.0246 & 0.0757 & 0.2127 &  & 11 & 213.41 & 10.33\% \\ 
\quad 100-999 & 0.1283 &  2,195,777  & 2,290.00  &  &  3,170.00  & 79.90\% &  & 0.0097 & 0.0253 & 0.0661 &  & 14 & 75.73 & 3.40\% \\ 
\quad +1000 & 0.0474 &  810,388  & 2,723.00  &  &  508.00  & 75.50\% &  & 0.0032 & 0.0087 & 0.0221 &  & 15 & 30.22 & 1.16\% \\ 
Gender x Education x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0037 &  83,776  & 0.00  &  &  3,250,000.00  & 98.60\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 2493.29 & (a) \\ 
\quad 1-2 & 0.1917 &  4,326,849  & 1,800.00  &  &  424,000.00  & 98.10\% &  & 0.1419 & 0.3679 & 0.8320 &  & 9 & 900.56 & 50.88\% \\ 
\quad 3-9 & 0.2087 &  4,709,531  & 1,908.00  &  &  241,000.00  & 95.90\% &  & 0.1254 & 0.2615 & 0.5459 &  & 9 & 678.95 & 36.16\% \\ 
\quad 10-99 & 0.3846 &  8,679,900  & 2,210.00  &  &  63,700.00  & 94.40\% &  & 0.0534 & 0.1158 & 0.2588 &  & 10 & 346.32 & 15.89\% \\ 
\quad 100-999 & 0.1715 &  3,871,290  & 2,558.00  &  &  12,000.00  & 94.30\% &  & 0.0203 & 0.0440 & 0.0937 &  & 10 & 150.32 & 6.04\% \\ 
\quad +1000 & 0.0398 &  897,250  & 3,175.00  &  &  2,870.00  & 94.20\% &  & 0.0076 & 0.0174 & 0.0408 &  & 10 & 73.51 & 2.38\% \\ 


==> tables/ame_table_b.tex <==
Age x Gender & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad 100-999 & 0.0001 &  3  & 1,779.00  &  &  15,000.00  & 87.00\% &  & 0.0688 & 0.0688 & 0.0688 &  & 11 & 166.99 & 9.38\% \\ 
\quad +1000 & 0.9999 &  44,941  & 2,176.00  &  &  5.39  & 23.50\% &  & 0.0004 & 0.0012 & 0.0062 &  & 164 & 2.99 & 0.15\% \\ 
Race x Ethnicity & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad 3-9 & 0.0002 &  7  & 2,335.00  &  &  307,000.00  & 97.10\% &  & 0.1820 & 0.3357 & 0.6261 &  & 9 & 766.30 & 46.42\% \\ 
\quad 10-99 & 0.0323 &  1,088  & 2,127.50  &  &  68,000.00  & 96.20\% &  & 0.0616 & 0.1201 & 0.3266 &  & 9 & 360.65 & 16.62\% \\ 
\quad 100-999 & 0.1687 &  5,685  & 2,225.00  &  &  8,170.00  & 94.70\% &  & 0.0133 & 0.0406 & 0.0979 &  & 10 & 124.03 & 5.57\% \\ 
\quad +1000 & 0.7989 &  26,928  & 2,508.50  &  &  140.00  & 75.30\% &  & 0.0004 & 0.0046 & 0.0302 &  & 15 & 15.86 & 0.61\% \\ 
Gender x Education & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad +1000 & 1.0000 &  22,472  & 2,844.00  &  &  63.60  & 94.70\% &  & 0.0011 & 0.0028 & 0.0080 &  & 10 & 10.94 & 0.38\% \\ 
Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0013 &  4,351  & 0.00  &  &  2,490,000.00  & 99.50\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 2182.38 & (a) \\ 
\quad 1-2 & 0.0859 &  288,667  & 2,135.00  &  &  6,710.00  & 0.00\% &  & 0.0000 & 0.0520 & 0.3027 &  & 9999 & 104.98 & 6.66\% \\ 
\quad 3-9 & 0.0252 &  84,593  & 1,520.00  &  &  9,030.00  & 0.00\% &  & 0.0196 & 0.0665 & 0.2977 &  & 9999 & 121.79 & 8.53\% \\ 
\quad 10-99 & 0.2632 &  884,129  & 1,969.00  &  &  6,060.00  & 44.00\% &  & 0.0147 & 0.0405 & 0.1292 &  & 46 & 101.22 & 5.26\% \\ 
\quad 100-999 & 0.4022 &  1,351,160  & 2,264.00  &  &  1,810.00  & 71.30\% &  & 0.0071 & 0.0197 & 0.0531 &  & 17 & 56.73 & 2.62\% \\ 
\quad +1000 & 0.2223 &  746,888  & 2,722.00  &  &  337.00  & 71.50\% &  & 0.0022 & 0.0071 & 0.0201 &  & 17 & 24.48 & 0.95\% \\ 
Age x Gender x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0016 &  69,616  & 0.00  &  &  2,790,000.00  & 99.70\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 2310.11 & (a) \\ 
\quad 1-2 & 0.2095 &  9,158,213  & 1,276.00  &  &  9,220.00  & 12.10\% &  & 0.0000 & 0.0852 & 0.4918 &  & 611 & 123.19 & 10.93\% \\ 
\quad 3-9 & 0.2357 &  10,301,188  & 1,469.00  &  &  18,700.00  & 73.50\% &  & 0.0298 & 0.0971 & 0.3096 &  & 16 & 182.80 & 12.97\% \\ 
\quad 10-99 & 0.3801 &  16,614,512  & 1,868.00  &  &  8,520.00  & 76.90\% &  & 0.0197 & 0.0532 & 0.1441 &  & 15 & 123.74 & 7.13\% \\ 
\quad 100-999 & 0.1457 &  6,367,152  & 2,383.00  &  &  2,040.00  & 77.40\% &  & 0.0079 & 0.0207 & 0.0526 &  & 15 & 60.55 & 2.77\% \\ 
\quad +1000 & 0.0274 &  1,197,767  & 3,152.00  &  &  481.00  & 73.30\% &  & 0.0029 & 0.0075 & 0.0191 &  & 16 & 29.32 & 1.01\% \\ 
Race x Ethnicity x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0027 &  51,636  & 0.00  &  &  6,010,000.00  & 99.90\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 3390.54 & (a) \\ 
\quad 1-2 & 0.3472 &  6,643,546  & 1,892.00  &  &  252,000.00  & 97.50\% &  & 0.0570 & 0.2777 & 0.7523 &  & 9 & 694.27 & 38.40\% \\ 
\quad 3-9 & 0.2153 &  4,119,278  & 2,009.00  &  &  132,000.00  & 93.90\% &  & 0.0580 & 0.1859 & 0.4701 &  & 10 & 498.54 & 25.51\% \\ 
\quad 10-99 & 0.2522 &  4,825,719  & 2,145.00  &  &  25,100.00  & 87.90\% &  & 0.0248 & 0.0748 & 0.2077 &  & 11 & 216.01 & 10.20\% \\ 
\quad 100-999 & 0.1328 &  2,541,058  & 2,324.00  &  &  2,840.00  & 80.90\% &  & 0.0087 & 0.0238 & 0.0624 &  & 13 & 71.95 & 3.21\% \\ 
\quad +1000 & 0.0499 &  955,663  & 2,763.00  &  &  430.00  & 75.90\% &  & 0.0027 & 0.0079 & 0.0212 &  & 15 & 27.80 & 1.06\% \\ 
Gender x Education x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0021 &  53,160  & 0.00  &  &  3,550,000.00  & 98.80\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 2605.83 & (a) \\ 
\quad 1-2 & 0.1652 &  4,096,117  & 1,803.00  &  &  451,000.00  & 98.20\% &  & 0.1473 & 0.3915 & 0.8583 &  & 9 & 928.79 & 54.15\% \\ 
\quad 3-9 & 0.1979 &  4,907,073  & 1,899.00  &  &  237,000.00  & 96.20\% &  & 0.1280 & 0.2628 & 0.5388 &  & 9 & 673.29 & 36.35\% \\ 
\quad 10-99 & 0.4035 &  10,007,726  & 2,205.00  &  &  57,100.00  & 94.70\% &  & 0.0499 & 0.1110 & 0.2480 &  & 10 & 327.89 & 15.22\% \\ 
\quad 100-999 & 0.1884 &  4,671,711  & 2,580.00  &  &  10,400.00  & 94.60\% &  & 0.0187 & 0.0411 & 0.0878 &  & 10 & 139.94 & 5.63\% \\ 
\quad +1000 & 0.0430 &  1,065,581  & 3,188.00  &  &  2,370.00  & 94.40\% &  & 0.0066 & 0.0160 & 0.0374 &  & 10 & 66.80 & 2.20\% \\ 


==> tables/ame_table_private.tex <==
\begin{landscape}
\begin{table}[htbp]
    \resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of Private Average Monthly Earnings ($EarnS$) by Table and Count}
\begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 15}{c}{} \\ 

\multicolumn{ 1}{c}{Table and $EmpS$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median Average} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Monthly Earnings} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Intervals Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
\multicolumn{15}{c}{\textbf{Private}} \\ 
\input{\MyPathtv/tables/ame_table_a.tex}
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Average Monthly Earnings is defined only over full-quarter jobs. It is calculated by taking the earnings for the reference quarter for full-quarter jobs and dividing by 3.  See the table on full-quarter employment for the relevent counts. Statistics are computed across all state-year-quarters within a table. The ``Private" category of establishments includes private only private establishments.. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for beginning of quarter employment, please see their respective equations in the accompanying text:  Average Monthly Earnings \ref{eq:z3pub}, Total Variation \ref{eq:tvz}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.  
 (a) Undefined value.
\end{tablenotes}
\label{tab:amepriv}
\end{threeparttable}
}%
\end{table}
\end{landscape}



==> tables/ame_table_total.tex <==
\begin{landscape}
\begin{table}[htbp]
    \resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of All Average Monthly Earnings ($EarnS$) by Table and Count}
\begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 15}{c}{} \\ 

\multicolumn{ 1}{c}{Table and $EmpS$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median Average} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Monthly Earnings} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Interval Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
\multicolumn{15}{c}{\textbf{All (Private plus State and Local)}} \\ 
\input{\MyPathtv/tables/ame_table_b.tex}
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Average Monthly Earnings is defined only over full-quarter jobs. It is calculated by taking the earnings for the reference quarter for full-quarter jobs and dividing by 3.  See the table on full-quarter employment for the relevent counts. Statistics are computed across all state-year-quarters within a table. The ``All" category of establishments includes private as well as state, and local government but excludes federal employment. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for beginning of quarter employment, please see their respective equations in the accompanying text:  Average Monthly Earnings \ref{eq:z3pub}, Total Variation \ref{eq:tvz}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.  
 (a) Undefined value.
\end{tablenotes}
\label{tab:ametot}
\end{threeparttable}
}%
\end{table}
\end{landscape}


==> tables/begemp_table_a.tex <==
Age x Gender &  & &  &  &  &  &  &  &  &  &  &  &  &  \\ 
\quad +1000 & 1.0000 &  45,712  & 61,308 &  & 5000.00 & 37.50\% &  & 0.0003 & 0.0011 & 0.0035 &  & 64 & 92 & 0.14\% \\ 
Race x Ethnicity &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\quad 3-9 & 0.0000 &  1  & 9 &  & 3.57 & 92.60\% &  & 0.2099 & 0.2099 & 0.2099 &  & 10 & 3 & 28.81\% \\ 
\quad 10-99 & 0.0282 &  968  & 47 &  & 36.80 & 95.90\% &  & 0.0783 & 0.1282 & 0.2729 &  & 9&8 & 17.73\% \\ 
\quad 100-999 & 0.1607 &  5,509  & 466 &  & 328.00 & 94.70\% &  & 0.0115 & 0.0427 & 0.0828 &  & 10&25 & 5.86\% \\ 
\quad +1000 & 0.8111 &  27,806  & 11,716 &  & 4000.00 & 83.20\% &  & 0.0002 & 0.0041 & 0.0241 &  & 13&85 & 0.55\% \\ 
Gender x Education &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\quad +1000 & 1.0000 &  22,856  & 132,437 &  & 136000.00 & 96.60\% &  & 0.0013 & 0.0031 & 0.0085 &  & 9 &510 & 0.42\% \\ 
Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
\quad zero measured value, after rounding & 0.0096 &  27,314  & 0 &  & 0.29 & 95.50\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
\quad 1-2 & 0.0001 &  313  & 2 &  & 0.37 & 66.90\% &  & 0.1425 & 0.3279 & 0.9000 &  & 20&1 & 43.45\% \\ 
\quad 3-9 & 0.0242 &  69,274  & 7 &  & 0.42 & 0.00\% &  & 0.0561 & 0.1009 & 0.3648 &  & 9999&1 & 12.93\% \\ 
\quad 10-99 & 0.2916 &  833,370  & 44 &  & 4.28 & 21.20\% &  & 0.0227 & 0.0499 & 0.1609 &  & 201&3 & 6.42\% \\ 
\quad 100-999 & 0.4286 &  1,225,043  & 283 &  & 51.40 & 71.10\% &  & 0.0102 & 0.0235 & 0.0586 &  & 17&10 & 3.14\% \\ 
\quad +1000 & 0.2459 &  702,856  & 2,936 &  & 747.00 & 78.70\% &  & 0.0024 & 0.0080 & 0.0199 &  & 14&37 & 1.08\% \\ 
Age x Gender x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
\quad zero measured value, after rounding & 0.2368 &  10,146,295  & 0 &  & 0.20 & 95.60\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
\quad 1-2 & 0.0051 &  217,085  & 2 &  & 0.33 & 69.70\% &  & 0.1409 & 0.2971 & 0.7099 &  & 18&1 & 39.52\% \\ 
\quad 3-9 & 0.2243 &  9,610,779  & 5 &  & 0.72 & 63.10\% &  & 0.0811 & 0.1641 & 0.3815 &  & 22&1 & 21.69\% \\ 
\quad 10-99 & 0.3624 &  15,526,526  & 26 &  & 4.98 & 72.80\% &  & 0.0365 & 0.0797 & 0.1786 &  & 17&3 & 10.63\% \\ 
\quad 100-999 & 0.1432 &  6,136,088  & 222 &  & 51.50 & 77.80\% &  & 0.0135 & 0.0296 & 0.0610 &  & 14&10 & 3.97\% \\ 
\quad +1000 & 0.0282 &  1,210,018  & 1,931 &  & 452.00 & 77.40\% &  & 0.0042 & 0.0101 & 0.0196 &  & 15&29 & 1.35\% \\ 
Race x Ethnicity x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
\quad zero measured value, after rounding & 0.6229 &  20,152,114  & 0 &  & 0.19 & 95.70\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
\quad 1-2 & 0.0052 &  168,667  & 2 &  & 0.66 & 92.30\% &  & 0.2579 & 0.6042 & 0.8972 &  & 10&1 & 82.90\% \\ 
\quad 3-9 & 0.1222 &  3,951,621  & 5 &  & 2.16 & 89.60\% &  & 0.1241 & 0.3040 & 0.5810 &  & 11&2 & 41.45\% \\ 
\quad 10-99 & 0.1465 &  4,740,254  & 26 &  & 9.16 & 85.80\% &  & 0.0395 & 0.1103 & 0.2619 &  & 12&4 & 14.96\% \\ 
\quad 100-999 & 0.0746 &  2,411,633  & 246 &  & 69.90 & 81.40\% &  & 0.0130 & 0.0310 & 0.0716 &  & 13&11 & 4.18\% \\ 
\quad +1000 & 0.0287 &  926,867  & 2,513 &  & 687.00 & 80.90\% &  & 0.0031 & 0.0093 & 0.0205 &  & 13&35 & 1.25\% \\ 
Gender x Education x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  & & \\ 
\quad zero measured value, after rounding & 0.1166 &  2,517,116  & 0 &  & 0.26 & 95.40\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
\quad 1-2 & 0.0055 &  118,679  & 2 &  & 1.34 & 93.80\% &  & 0.4257 & 0.6500 & 0.9392 &  & 10&2 & 89.19\% \\ 
\quad 3-9 & 0.2150 &  4,638,908  & 5 &  & 3.87 & 93.50\% &  & 0.2365 & 0.3763 & 0.6062 &  & 10&3 & 51.64\% \\ 
\quad 10-99 & 0.4195 &  9,052,346  & 28 &  & 21.00 & 93.60\% &  & 0.0857 & 0.1620 & 0.2946 &  & 10&6 & 22.23\% \\ 
\quad 100-999 & 0.1959 &  4,228,095  & 232 &  & 183.00 & 93.90\% &  & 0.0288 & 0.0563 & 0.0957 &  & 10&19 & 7.73\% \\ 
\quad +1000 & 0.0475 &  1,025,888  & 2,045 &  & 1670.00 & 94.20\% &  & 0.0086 & 0.0191 & 0.0315 &  & 10&56 & 2.62\% \\ 



==> tables/begemp_table_ab.tex <==
Age x Gender &  & &  &  &  &  &  &  &  &  &  &  &  &  \\ 
+1000 & 1.0000 &  45,712  & 61,308 &  & 5000.00 & 37.50\% &  & 0.0003 & 0.0011 & 0.0035 &  & 64 & 92 & 0.14\% \\ 
Race x Ethnicity &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
3-9 & 0.0000 &  1  & 9 &  & 3.57 & 92.60\% &  & 0.2099 & 0.2099 & 0.2099 &  & 10 & 3 & 28.81\% \\ 
10-99 & 0.0282 &  968  & 47 &  & 36.80 & 95.90\% &  & 0.0783 & 0.1282 & 0.2729 &  & 9&8 & 17.73\% \\ 
100-999 & 0.1607 &  5,509  & 466 &  & 328.00 & 94.70\% &  & 0.0115 & 0.0427 & 0.0828 &  & 10&25 & 5.86\% \\ 
+1000 & 0.8111 &  27,806  & 11,716 &  & 4000.00 & 83.20\% &  & 0.0002 & 0.0041 & 0.0241 &  & 13&85 & 0.55\% \\ 
Gender x Education &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
+1000 & 1.0000 &  22,856  & 132,437 &  & 136000.00 & 96.60\% &  & 0.0013 & 0.0031 & 0.0085 &  & 9 &510 & 0.42\% \\ 
Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  & \\ 
zero measured value, after rounding & 0.0096 &  27,314  & 0 &  & 0.29 & 95.50\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
1-2 & 0.0001 &  313  & 2 &  & 0.37 & 66.90\% &  & 0.1425 & 0.3279 & 0.9000 &  & 20&1 & 43.45\% \\ 
3-9 & 0.0242 &  69,274  & 7 &  & 0.42 & 0.00\% &  & 0.0561 & 0.1009 & 0.3648 &  & 9999&1 & 12.93\% \\ 
10-99 & 0.2916 &  833,370  & 44 &  & 4.28 & 21.20\% &  & 0.0227 & 0.0499 & 0.1609 &  & 201&3 & 6.42\% \\ 
100-999 & 0.4286 &  1,225,043  & 283 &  & 51.40 & 71.10\% &  & 0.0102 & 0.0235 & 0.0586 &  & 17&10 & 3.14\% \\ 
+1000 & 0.2459 &  702,856  & 2,936 &  & 747.00 & 78.70\% &  & 0.0024 & 0.0080 & 0.0199 &  & 14&37 & 1.08\% \\ 
Age x Gender x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
zero measured value, after rounding & 0.2368 &  10,146,295  & 0 &  & 0.20 & 95.60\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
1-2 & 0.0051 &  217,085  & 2 &  & 0.33 & 69.70\% &  & 0.1409 & 0.2971 & 0.7099 &  & 18&1 & 39.52\% \\ 
3-9 & 0.2243 &  9,610,779  & 5 &  & 0.72 & 63.10\% &  & 0.0811 & 0.1641 & 0.3815 &  & 22&1 & 21.69\% \\ 
10-99 & 0.3624 &  15,526,526  & 26 &  & 4.98 & 72.80\% &  & 0.0365 & 0.0797 & 0.1786 &  & 17&3 & 10.63\% \\ 
100-999 & 0.1432 &  6,136,088  & 222 &  & 51.50 & 77.80\% &  & 0.0135 & 0.0296 & 0.0610 &  & 14&10 & 3.97\% \\ 
+1000 & 0.0282 &  1,210,018  & 1,931 &  & 452.00 & 77.40\% &  & 0.0042 & 0.0101 & 0.0196 &  & 15&29 & 1.35\% \\ 
Race x Ethnicity x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
zero measured value, after rounding & 0.6229 &  20,152,114  & 0 &  & 0.19 & 95.70\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
1-2 & 0.0052 &  168,667  & 2 &  & 0.66 & 92.30\% &  & 0.2579 & 0.6042 & 0.8972 &  & 10&1 & 82.90\% \\ 
3-9 & 0.1222 &  3,951,621  & 5 &  & 2.16 & 89.60\% &  & 0.1241 & 0.3040 & 0.5810 &  & 11&2 & 41.45\% \\ 
10-99 & 0.1465 &  4,740,254  & 26 &  & 9.16 & 85.80\% &  & 0.0395 & 0.1103 & 0.2619 &  & 12&4 & 14.96\% \\ 
100-999 & 0.0746 &  2,411,633  & 246 &  & 69.90 & 81.40\% &  & 0.0130 & 0.0310 & 0.0716 &  & 13&11 & 4.18\% \\ 
+1000 & 0.0287 &  926,867  & 2,513 &  & 687.00 & 80.90\% &  & 0.0031 & 0.0093 & 0.0205 &  & 13&35 & 1.25\% \\ 
Gender x Education x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  & & \\ 
zero measured value, after rounding & 0.1166 &  2,517,116  & 0 &  & 0.26 & 95.40\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
1-2 & 0.0055 &  118,679  & 2 &  & 1.34 & 93.80\% &  & 0.4257 & 0.6500 & 0.9392 &  & 10&2 & 89.19\% \\ 
3-9 & 0.2150 &  4,638,908  & 5 &  & 3.87 & 93.50\% &  & 0.2365 & 0.3763 & 0.6062 &  & 10&3 & 51.64\% \\ 
10-99 & 0.4195 &  9,052,346  & 28 &  & 21.00 & 93.60\% &  & 0.0857 & 0.1620 & 0.2946 &  & 10&6 & 22.23\% \\ 
100-999 & 0.1959 &  4,228,095  & 232 &  & 183.00 & 93.90\% &  & 0.0288 & 0.0563 & 0.0957 &  & 10&19 & 7.73\% \\ 
+1000 & 0.0475 &  1,025,888  & 2,045 &  & 1670.00 & 94.20\% &  & 0.0086 & 0.0191 & 0.0315 &  & 10&56 & 2.62\% \\ 
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
 \textbf{B: All (Private Plus State and Local)} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{}\textbf{} & \textbf{} \\ 
  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  Age x Gender &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
  +1000 & 1.0000 &  45,712  & 70,233 &  & 5300.00 & 37.00\% &  & 0.0003 & 0.0010 & 0.0032 &  & 65&94 & 0.13\% \\ 
  Race x Ethnicity &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
  10-99 & 0.0258 &  883  & 51 &  & 39.50 & 96.50\% &  & 0.0793 & 0.1277 & 0.2664 &  & 9&9 & 17.66\% \\ 
  100-999 & 0.1489 &  5,105  & 454 &  & 326.00 & 95.10\% &  & 0.0198 & 0.0430 & 0.0830 &  & 9&25 & 5.95\% \\ 
  +1000 & 0.8253 &  28,296  & 12,858 &  & 4340.00 & 84.60\% &  & 0.0001 & 0.0038 & 0.0237 &  & 12&89 & 0.52\% \\ 
  Gender x Education &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
  +1000 & 1.0000 &  22,856  & 161,812 &  & 162000.00 & 96.80\% &  & 0.0012 & 0.0028 & 0.0079 &  & 9 &557 & 0.39\% \\ 
  Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
  zero measured value, after rounding & 0.0056 &  17,598  & 0 &  & 0.28 & 95.50\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
  1-2 & 0.0001 &  257  & 2 &  & 0.44 & 78.30\% &  & 0.1443 & 0.3592 & 0.8972 &  & 14&1 & 48.31\% \\ 
  3-9 & 0.0203 &  63,664  & 7 &  & 0.43 & 0.00\% &  & 0.0546 & 0.1022 & 0.3814 &  & 9999&1 & 13.09\% \\ 
  10-99 & 0.2633 &  827,121  & 45 &  & 5.06 & 50.30\% &  & 0.0223 & 0.0529 & 0.1643 &  & 35&3 & 6.91\% \\ 
  100-999 & 0.4464 &  1,402,205  & 295 &  & 55.70 & 74.70\% &  & 0.0099 & 0.0240 & 0.0590 &  & 16&10 & 3.20\% \\ 
  +1000 & 0.2643 &  830,357  & 2,875 &  & 711.00 & 79.30\% &  & 0.0023 & 0.0080 & 0.0197 &  & 14&36 & 1.07\% \\ 
  Age x Gender x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
  zero measured value, after rounding & 0.2011 &  9,317,087  & 0 &  & 0.20 & 95.80\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
  1-2 & 0.0051 &  234,090  & 2 &  & 0.36 & 74.20\% &  & 0.1371 & 0.3156 & 0.7273 &  & 16&1 & 42.19\% \\ 
  3-9 & 0.2246 &  10,406,647  & 5 &  & 0.77 & 67.90\% &  & 0.0794 & 0.1675 & 0.3873 &  & 19&1 & 22.24\% \\ 
  10-99 & 0.3842 &  17,797,008  & 27 &  & 4.99 & 74.40\% &  & 0.0351 & 0.0791 & 0.1793 &  & 16&3 & 10.58\% \\ 
  100-999 & 0.1547 &  7,165,326  & 222 &  & 48.90 & 77.90\% &  & 0.0131 & 0.0288 & 0.0603 &  & 14&9 & 3.87\% \\ 
  +1000 & 0.0303 &  1,405,442  & 1,945 &  & 437.00 & 77.60\% &  & 0.0039 & 0.0097 & 0.0192 &  & 14&28 & 1.31\% \\ 
  Race x Ethnicity x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
  zero measured value, after rounding & 0.6023 &  20,718,981  & 0 &  & 0.19 & 96.00\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
  1-2 & 0.0056 &  191,678  & 2 &  & 0.67 & 92.70\% &  & 0.2632 & 0.6050 & 0.9028 &  & 10&1 & 83.01\% \\ 
  3-9 & 0.1288 &  4,431,864  & 5 &  & 2.16 & 90.10\% &  & 0.1256 & 0.3044 & 0.5799 &  & 11&2 & 41.50\% \\ 
  10-99 & 0.1514 &  5,208,590  & 26 &  & 9.27 & 86.80\% &  & 0.0402 & 0.1115 & 0.2610 &  & 11&4 & 15.20\% \\ 
  100-999 & 0.0805 &  2,767,906  & 251 &  & 69.40 & 82.00\% &  & 0.0126 & 0.0307 & 0.0710 &  & 13&11 & 4.15\% \\ 
  +1000 & 0.0314 &  1,081,496  & 2,506 &  & 673.00 & 81.30\% &  & 0.0030 & 0.0091 & 0.0204 &  & 13&35 & 1.23\% \\ 
  Gender x Education x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
  zero measured value, after rounding & 0.0870 &  2,055,422  & 0 &  & 0.26 & 95.70\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
  1-2 & 0.0049 &  114,711  & 2 &  & 1.37 & 94.20\% &  & 0.4269 & 0.6496 & 0.9421 &  & 10&2 & 89.14\% \\ 
  3-9 & 0.2033 &  4,805,343  & 5 &  & 3.93 & 93.90\% &  & 0.2359 & 0.3758 & 0.6065 &  & 10&3 & 51.56\% \\ 
  10-99 & 0.4392 &  10,378,260  & 29 &  & 21.50 & 94.00\% &  & 0.0846 & 0.1597 & 0.2935 &  & 10&6 & 21.91\% \\ 
  100-999 & 0.2146 &  5,070,981  & 231 &  & 180.00 & 94.10\% &  & 0.0286 & 0.0561 & 0.0953 &  & 10&18 & 7.69\% \\ 
  +1000 & 0.0511 &  1,207,342  & 2,051 &  & 1660.00 & 94.40\% &  & 0.0085 & 0.0190 & 0.0313 &  & 10&56 & 2.60\% \\ 


==> tables/begemp_table_b.tex <==
Age x Gender &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
\quad +1000 & 1.0000 &  45,712  & 70,233 &  & 5300.00 & 37.00\% &  & 0.0003 & 0.0010 & 0.0032 &  & 65&94 & 0.13\% \\ 
Race x Ethnicity &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
\quad  10-99 & 0.0258 &  883  & 51 &  & 39.50 & 96.50\% &  & 0.0793 & 0.1277 & 0.2664 &  & 9&9 & 17.66\% \\ 
\quad  100-999 & 0.1489 &  5,105  & 454 &  & 326.00 & 95.10\% &  & 0.0198 & 0.0430 & 0.0830 &  & 9&25 & 5.95\% \\ 
\quad  +1000 & 0.8253 &  28,296  & 12,858 &  & 4340.00 & 84.60\% &  & 0.0001 & 0.0038 & 0.0237 &  & 12&89 & 0.52\% \\ 
Gender x Education &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
\quad  +1000 & 1.0000 &  22,856  & 161,812 &  & 162000.00 & 96.80\% &  & 0.0012 & 0.0028 & 0.0079 &  & 9 &557 & 0.39\% \\ 
Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
\quad  zero measured value, after rounding & 0.0056 &  17,598  & 0 &  & 0.28 & 95.50\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
\quad  1-2 & 0.0001 &  257  & 2 &  & 0.44 & 78.30\% &  & 0.1443 & 0.3592 & 0.8972 &  & 14&1 & 48.31\% \\ 
\quad  3-9 & 0.0203 &  63,664  & 7 &  & 0.43 & 0.00\% &  & 0.0546 & 0.1022 & 0.3814 &  & 9999&1 & 13.09\% \\ 
\quad  10-99 & 0.2633 &  827,121  & 45 &  & 5.06 & 50.30\% &  & 0.0223 & 0.0529 & 0.1643 &  & 35&3 & 6.91\% \\ 
\quad  100-999 & 0.4464 &  1,402,205  & 295 &  & 55.70 & 74.70\% &  & 0.0099 & 0.0240 & 0.0590 &  & 16&10 & 3.20\% \\ 
\quad  +1000 & 0.2643 &  830,357  & 2,875 &  & 711.00 & 79.30\% &  & 0.0023 & 0.0080 & 0.0197 &  & 14&36 & 1.07\% \\ 
  Age x Gender x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
\quad  zero measured value, after rounding & 0.2011 &  9,317,087  & 0 &  & 0.20 & 95.80\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
\quad  1-2 & 0.0051 &  234,090  & 2 &  & 0.36 & 74.20\% &  & 0.1371 & 0.3156 & 0.7273 &  & 16&1 & 42.19\% \\ 
\quad  3-9 & 0.2246 &  10,406,647  & 5 &  & 0.77 & 67.90\% &  & 0.0794 & 0.1675 & 0.3873 &  & 19&1 & 22.24\% \\ 
\quad  10-99 & 0.3842 &  17,797,008  & 27 &  & 4.99 & 74.40\% &  & 0.0351 & 0.0791 & 0.1793 &  & 16&3 & 10.58\% \\ 
\quad  100-999 & 0.1547 &  7,165,326  & 222 &  & 48.90 & 77.90\% &  & 0.0131 & 0.0288 & 0.0603 &  & 14&9 & 3.87\% \\ 
\quad  +1000 & 0.0303 &  1,405,442  & 1,945 &  & 437.00 & 77.60\% &  & 0.0039 & 0.0097 & 0.0192 &  & 14&28 & 1.31\% \\ 
Race x Ethnicity x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
\quad  zero measured value, after rounding & 0.6023 &  20,718,981  & 0 &  & 0.19 & 96.00\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
\quad  1-2 & 0.0056 &  191,678  & 2 &  & 0.67 & 92.70\% &  & 0.2632 & 0.6050 & 0.9028 &  & 10&1 & 83.01\% \\ 
\quad  3-9 & 0.1288 &  4,431,864  & 5 &  & 2.16 & 90.10\% &  & 0.1256 & 0.3044 & 0.5799 &  & 11&2 & 41.50\% \\ 
\quad  10-99 & 0.1514 &  5,208,590  & 26 &  & 9.27 & 86.80\% &  & 0.0402 & 0.1115 & 0.2610 &  & 11&4 & 15.20\% \\ 
\quad  100-999 & 0.0805 &  2,767,906  & 251 &  & 69.40 & 82.00\% &  & 0.0126 & 0.0307 & 0.0710 &  & 13&11 & 4.15\% \\ 
\quad  +1000 & 0.0314 &  1,081,496  & 2,506 &  & 673.00 & 81.30\% &  & 0.0030 & 0.0091 & 0.0204 &  & 13&35 & 1.23\% \\ 
Gender x Education x Industry x County &  &  &  &  &  &  &  &  &  &  &  &  &  &\\ 
\quad  zero measured value, after rounding & 0.0870 &  2,055,422  & 0 &  & 0.26 & 95.70\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\ 
\quad  1-2 & 0.0049 &  114,711  & 2 &  & 1.37 & 94.20\% &  & 0.4269 & 0.6496 & 0.9421 &  & 10&2 & 89.14\% \\ 
\quad  3-9 & 0.2033 &  4,805,343  & 5 &  & 3.93 & 93.90\% &  & 0.2359 & 0.3758 & 0.6065 &  & 10&3 & 51.56\% \\ 
\quad  10-99 & 0.4392 &  10,378,260  & 29 &  & 21.50 & 94.00\% &  & 0.0846 & 0.1597 & 0.2935 &  & 10&6 & 21.91\% \\ 
\quad  100-999 & 0.2146 &  5,070,981  & 231 &  & 180.00 & 94.10\% &  & 0.0286 & 0.0561 & 0.0953 &  & 10&18 & 7.69\% \\ 
\quad  +1000 & 0.0511 &  1,207,342  & 2,051 &  & 1660.00 & 94.40\% &  & 0.0085 & 0.0190 & 0.0313 &  & 10&56 & 2.60\% \\ 


==> tables/begemp_table_private.tex <==
\begin{landscape}
\begin{table}[htbp]
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of Private Beginning-of-Quarter Employment ($Emp$) by Table and Count}
    \begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 1}{c}{Table and $Emp$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Count} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Intervals Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
%
\multicolumn{15}{c}{\textbf{Private}} \\ 
%\input{\MyPathtv/tables/begemp_table_ab.tex}
\input{\MyPathtv/tables/begemp_table_a.tex}
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Beginning-of-quarter employment is defined as all jobs held by a worker at the same establishment during the quarter and during the previous quarter. Statistics are computed across all state-year-quarters within a table. The ``Private" category of establishments includes only private establishments. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for beginning of quarter employment, please see their respective equations in the accompanying text:  Count \ref{eq:theb}, Total Variation \ref{eq:tvc}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.  
 (a) Undefined value.
\end{tablenotes}
\label{tab:empprivate}
\end{threeparttable}
}%
\end{table}
\end{landscape}



==> tables/begemp_table_total.tex <==
\begin{landscape}
\begin{table}[htbp]
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of All Beginning-of-Quarter Employment ($Emp$) by Table and Count}
    \begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 1}{c}{Table and $Emp$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Count} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Intervals Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
%Panel B 
        \multicolumn{15}{c}{\textbf{All (Private plus State and Local)}} \\ 
%\input{\MyPathtv/tables/begemp_table_ab.tex}
\input{\MyPathtv/tables/begemp_table_b.tex}
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Beginning-of-quarter employment is defined as all jobs held by a worker at the same establishment during the quarter and during the previous quarter. Statistics are computed across all state-year-quarters within a table. The ``All" category of establishments includes private as well as state and local government but excludes federal employment. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for beginning of quarter employment, please see their respective equations in the accompanying text:  Count \ref{eq:theb}, Total Variation \ref{eq:tvc}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.  
(a) Undefined value.
\end{tablenotes}
\label{tab:emp}
\end{threeparttable}
}%
\end{table}
\end{landscape}



==> tables/betvar_b.tex <==
\begin{table}[htbp] 
\begin{center}
%\resizebox{\linewidth}{!}{
\scalebox{0.70}{
    \begin{threeparttable}
    \caption{Between Variance of Beginning-of-Quarter ($B$) Population Counts}
    \begin{tabular}{lrrrrr} \toprule 
    & & \multicolumn{4}{c}{Coefficient of Variation}  \\ \cmidrule{3-6} 
 & \multicolumn{ 1}{c}{Cell Count} & \multicolumn{ 1}{c}{Mean} & \multicolumn{ 1}{c}{Std Dev} &   \multicolumn{ 1}{c}{Minimum} & \multicolumn{ 1}{c}{Maximum} \\ \midrule 
    \multicolumn{6}{c}{\textbf{A: Establishment Type and Age Range}} \\ 
    {\it Population}    & & & & & \\
    \quad All Valid QWI Ages, All Establishments      &2,957  &   1.059E-05 &  6.175E-06  & 1.738E-06 &  5.334E-05 \\
\quad All Valid QWI Ages, Private Establishments      &2,957  &   1.187E-05 &  6.911E-06  & 1.984E-06 &  6.670E-05 \\

    & & & & & \\
    \multicolumn{6}{c}{\textbf{B: State}} \\ 
    {\it Postal Code}    & & & & & \\
\quad    AK  & 188  &  6.521E-05 &  5.021E-05 &  6.874E-06 &  2.234E-04\\
\quad    AL  & 172  &  3.040E-05 &  2.319E-05 &  3.695E-06 &  8.993E-05\\
\quad    AR  & 148  &  3.248E-05 &  2.201E-05 &  7.540E-06 &  7.745E-05\\
\quad    AZ  & 124  &  4.091E-05 &  3.357E-05 &  6.086E-06 &  1.385E-04\\
\quad    CA  & 324  &  2.463E-05 &  2.074E-05 &  2.581E-06 &  9.171E-05\\
\quad    CT  & 252  &  3.362E-05 &  2.643E-05 &  5.869E-06 &  1.417E-04\\
\quad    DC  & 104  &  8.532E-05 &  5.890E-05 &  1.611E-05 &  1.984E-04\\
\quad    DE  & 212  &  6.939E-05 &  5.802E-05 &  8.776E-06 &  2.319E-04\\
\quad    FL  & 304  &  1.812E-05 &  1.435E-05 &  2.625E-06 &  7.097E-05\\
\quad    GA  & 220  &  3.069E-05 &  2.497E-05 &  3.249E-06 &  1.027E-04\\
\quad    HI  & 256  &  4.458E-05 &  4.397E-05 &  5.854E-06 &  2.369E-04\\
\quad    IA  & 208  &  2.941E-05 &  2.218E-05 &  4.336E-06 &  1.009E-04\\
\quad    ID  & 332  &  6.875E-05 &  5.681E-05 &  6.696E-06 &  3.292E-04\\
\quad    IL  & 348  &  2.606E-05 &  2.101E-05 &  2.660E-06 &  7.849E-05\\
\quad    IN  & 220  &  2.383E-05 &  1.818E-05 &  2.140E-06 &  6.173E-05\\
\quad    KS  & 300  &  3.931E-05 &  3.122E-05 &  5.063E-06 &  1.262E-04\\
\quad    KY  & 172  &  2.659E-05 &  1.998E-05 &  3.718E-06 &  7.896E-05\\
\quad    LA  & 268  &  2.138E-05 &  1.482E-05 &  4.411E-06 &  6.201E-05\\
\quad    MD  & 348  &  3.166E-05 &  2.787E-05 &  3.609E-06 &  1.276E-04\\
\quad    ME  & 248  &  3.069E-05 &  2.227E-05 &  5.408E-06 &  9.439E-05\\
\quad    MI  & 180  &  1.896E-05 &  1.498E-05 &  3.122E-06 &  5.559E-05\\
\quad    MN  & 276  &  2.373E-05 &  1.933E-05 &  3.230E-06 &  6.993E-05\\
\quad    MO  & 268  &  2.291E-05 &  1.892E-05 &  2.885E-06 &  6.340E-05\\
\quad    MS  & 132  &  3.457E-05 &  2.448E-05 &  5.182E-06 &  8.206E-05\\
\quad    MT  & 300  &  4.375E-05 &  3.270E-05 &  7.252E-06 &  1.399E-04\\
\quad    ND  & 220  &  4.782E-05 &  3.732E-05 &  6.366E-06 &  1.632E-04\\
\quad    NE  & 204  &  3.910E-05 &  3.037E-05 &  6.833E-06 &  1.090E-04\\
\quad    NH  & 140  &  4.042E-05 &  2.809E-05 &  7.394E-06 &  9.946E-05\\
\quad    NJ  & 252  &  2.982E-05 &  2.341E-05 &  3.494E-06 &  1.275E-04\\
\quad    NM  & 260  &  7.141E-05 &  6.564E-05 &  6.204E-06 &  3.728E-04\\
\quad    NV  & 220  &  6.333E-05 &  5.146E-05 &  6.337E-06 &  1.739E-04\\
\quad    NY  & 188  &  2.334E-05 &  2.095E-05 &  2.948E-06 &  1.143E-04\\
\quad    OH  & 188  &  1.475E-05 &  1.147E-05 &  2.241E-06 &  4.309E-05\\
\quad    OK  & 188  &  4.435E-05 &  3.440E-05 &  4.895E-06 &  1.131E-04\\
\quad    OR  & 332  &  3.848E-05 &  2.973E-05 &  5.838E-06 &  1.269E-04\\
\quad    PA  & 236  &  1.181E-05 &  8.594E-06 &  1.738E-06 &  3.660E-05\\
\quad    RI  & 268  &  6.231E-05 &  4.507E-05 &  6.479E-06 &  1.753E-04\\
\quad    SC  & 220  &  3.604E-05 &  2.772E-05 &  4.599E-06 &  9.803E-05\\
\quad    SD  & 220  &  5.157E-05 &  4.009E-05 &  6.421E-06 &  1.497E-04\\
\quad    TN  & 220  &  2.394E-05 &  1.913E-05 &  2.935E-06 &  8.213E-05\\
\quad    TX  & 268  &  1.945E-05 &  1.583E-05 &  2.284E-06 &  7.985E-05\\
\quad    UT  & 196  &  6.618E-05 &  5.351E-05 &  7.202E-06 &  1.792E-04\\
\quad    VA  & 220  &  2.814E-05 &  2.341E-05 &  4.003E-06 &  1.111E-04\\
\quad    VT  & 188  &  4.439E-05 &  3.280E-05 &  5.941E-06 &  1.317E-04\\
\quad    WA  & 348  &  3.202E-05 &  2.560E-05 &  4.074E-06 &  9.715E-05\\
\quad    WI  & 348  &  2.128E-05 &  1.751E-05 &  1.960E-06 &  7.021E-05\\
\quad    WV  & 236  &  2.298E-05 &  1.554E-05 &  3.872E-06 &  7.009E-05\\
\quad    WY  & 172  &  8.874E-05 &  6.879E-05 &  1.586E-05 &  2.701E-04\\

\bottomrule    
\end{tabular}

\footnotesize
\begin{tablenotes}
\item {\it Notes}: There is small amount of between-implicate variance of state counts for beginning-of-quarter  employment. We summarize the between variance using the coefficient of variation defined as the square root of the between-implicate variance divided by the average between-implicate weighted counts. Panel A summarizes the coefficient of variation for the between variance for the four different types of ownership type and age populations. The summary is taken across all state-year-quarters. Panel B summarizes the coefficient of variation for all states across all year, quarters, and ownership types and age range combinations.  
\end{tablenotes}
\label{tab:betb}
\end{threeparttable}
}%
\end{center}
\end{table}


==> tables/betvar_f.tex <==
\begin{table}[htbp] 
\begin{center}
%\resizebox{\linewidth}{!}{
\scalebox{0.70}{
    \begin{threeparttable}
    \caption{Between Variance of Full-Quarter ($F$) Population Counts}
    \begin{tabular}{lrrrrr} \toprule 
    & & \multicolumn{4}{c}{Coefficient of Variation}  \\ \cmidrule{3-6} 
 & \multicolumn{ 1}{c}{Cell Count} & \multicolumn{ 1}{c}{Mean} & \multicolumn{ 1}{c}{Std Dev} &   \multicolumn{ 1}{c}{Minimum} & \multicolumn{ 1}{c}{Maximum} \\ \midrule 
    \multicolumn{6}{c}{\textbf{A: Establishment Type and Age Range}} \\ 
    {\it Population}    & & & & & \\
\quad All Valid QWI Ages, All Establishments      &  2,957 &  1.027E-05 &  5.891E-06 &  2.149E-06 &   5.356E-05 \\
\quad All Valid QWI Ages, Private Establishments  &  2,957 & 1.152E-05  & 6.592E-06  & 1.990E-06  & 5.403E-05   \\
    
    & & & & & \\
    \multicolumn{6}{c}{\textbf{B: State}} \\ 
    {\it Postal Code}    & & & & & \\
\quad AK &  188  &  5.625E-05 &  4.128E-05 &  7.485E-06 &  1.601E-04\\
\quad AL &  172  &  2.873E-05 &  2.214E-05 &  3.299E-06 &  8.659E-05\\
\quad AR &  148  &  3.144E-05 &  2.094E-05 &  6.305E-06 &  7.746E-05\\
\quad AZ &  124  &  4.139E-05 &  3.343E-05 &  5.211E-06 &  1.432E-04\\
\quad CA &  324  &  2.273E-05 &  1.914E-05 &  2.422E-06 &  8.591E-05\\
\quad CT &  252  &  3.258E-05 &  2.605E-05 &  5.610E-06 &  1.371E-04\\
\quad DC &  104  &  8.303E-05 &  5.866E-05 &  1.708E-05 &  2.181E-04\\
\quad DE &  212  &  6.386E-05 &  5.424E-05 &  5.393E-06 &  2.005E-04\\
\quad FL &  304  &  1.645E-05 &  1.296E-05 &  2.559E-06 &  6.220E-05\\
\quad GA &  220  &  2.916E-05 &  2.281E-05 &  3.254E-06 &  8.538E-05\\
\quad HI &  256  &  4.090E-05 &  4.112E-05 &  5.684E-06 &  2.272E-04\\
\quad IA &  208  &  2.801E-05 &  2.095E-05 &  4.748E-06 &  7.924E-05\\
\quad ID &  332  &  6.090E-05 &  4.640E-05 &  8.729E-06 &  1.853E-04\\
\quad IL &  348  &  2.404E-05 &  1.901E-05 &  2.408E-06 &  6.948E-05\\
\quad IN &  220  &  2.254E-05 &  1.722E-05 &  3.352E-06 &  6.253E-05\\
\quad KS &  300  &  3.776E-05 &  3.054E-05 &  5.557E-06 &  1.261E-04\\
\quad KY &  172  &  2.588E-05 &  1.884E-05 &  3.681E-06 &  8.234E-05\\
\quad LA &  268  &  2.087E-05 &  1.429E-05 &  3.630E-06 &  5.697E-05\\
\quad MD &  348  &  2.926E-05 &  2.510E-05 &  3.640E-06 &  1.148E-04\\
\quad ME &  248  &  2.783E-05 &  1.945E-05 &  4.771E-06 &  8.563E-05\\
\quad MI &  180  &  1.626E-05 &  1.206E-05 &  2.406E-06 &  4.997E-05\\
\quad MN &  276  &  2.264E-05 &  1.861E-05 &  2.661E-06 &  6.325E-05\\
\quad MO &  268  &  2.164E-05 &  1.737E-05 &  3.001E-06 &  6.110E-05\\
\quad MS &  132  &  3.374E-05 &  2.393E-05 &  4.847E-06 &  9.564E-05\\
\quad MT &  300  &  4.097E-05 &  2.925E-05 &  7.754E-06 &  1.329E-04\\
\quad ND &  220  &  4.407E-05 &  3.356E-05 &  5.709E-06 &  1.191E-04\\
\quad NE &  204  &  3.838E-05 &  2.992E-05 &  4.032E-06 &  1.109E-04\\
\quad NH &  140  &  3.957E-05 &  2.731E-05 &  6.623E-06 &  9.685E-05\\
\quad NJ &  252  &  2.814E-05 &  2.202E-05 &  4.148E-06 &  9.915E-05\\
\quad NM &  260  &  6.823E-05 &  5.648E-05 &  6.973E-06 &  2.258E-04\\
\quad NV &  220  &  5.935E-05 &  4.752E-05 &  6.652E-06 &  1.766E-04\\
\quad NY &  188  &  2.177E-05 &  1.894E-05 &  2.341E-06 &  9.451E-05\\
\quad OH &  188  &  1.402E-05 &  1.088E-05 &  2.160E-06 &  3.793E-05\\
\quad OK &  188  &  4.342E-05 &  3.421E-05 &  3.832E-06 &  1.146E-04\\
\quad OR &  332  &  3.542E-05 &  2.710E-05 &  5.739E-06 &  1.056E-04\\
\quad PA &  236  &  1.094E-05 &  7.845E-06 &  1.990E-06 &  3.553E-05\\
\quad RI &  268  &  5.713E-05 &  4.069E-05 &  9.523E-06 &  1.553E-04\\
\quad SC &  220  &  3.390E-05 &  2.587E-05 &  4.492E-06 &  1.016E-04\\
\quad SD &  220  &  4.917E-05 &  3.734E-05 &  7.047E-06 &  1.459E-04\\
\quad TN &  220  &  2.221E-05 &  1.741E-05 &  2.674E-06 &  6.856E-05\\
\quad TX &  268  &  1.757E-05 &  1.413E-05 &  2.003E-06 &  6.805E-05\\
\quad UT &  196  &  6.683E-05 &  5.510E-05 &  7.998E-06 &  1.977E-04\\
\quad VA &  220  &  2.636E-05 &  2.214E-05 &  3.717E-06 &  1.089E-04\\
\quad VT &  188  &  4.051E-05 &  2.909E-05 &  7.829E-06 &  1.249E-04\\
\quad WA &  348  &  2.724E-05 &  2.122E-05 &  3.714E-06 &  7.521E-05\\
\quad WI &  348  &  2.052E-05 &  1.673E-05 &  3.026E-06 &  6.773E-05\\
\quad WV &  236  &  2.199E-05 &  1.394E-05 &  3.598E-06 &  6.286E-05\\
\quad WY &  172  &  8.041E-05 &  6.154E-05 &  1.300E-05 &  2.730E-04\\

\bottomrule    
\end{tabular}
%}%
\footnotesize
\begin{tablenotes}
\item {\it Notes}: There is small amount of between-implicate variance of state counts for full-quarter employment. We summarize the between variance using the coefficient of variation defined as the square root of the between-implicate variance divided by the average between-implicate weighted counts. Panel A summarizes the coefficient of variation for the between variance for the four different types of ownership type and age populations. The summary is taken across all state-year-quarters. Panel B summarizes the coefficient of variation for all states across all year, quarters, and ownership types and age range combinations. 
\end{tablenotes}
\label{tab:betf}
\end{threeparttable}
}%
\end{center}
\end{table}


==> tables/d_sample_state.tex <==
\begin{table}[htbp]
\begin{center}
\resizebox{\linewidth}{!}{
%\scalebox{0.70}{
    \begin{threeparttable}
        \caption{Comparison of QWI Variables for the Decennial Sample (D Sample): Actual vs. Imputed Education}
    \begin{tabular}{lrrrrrrrrrrr} \toprule
        & & & & & & & & & & \multicolumn{2}{c}{Average Full-quarter}  \\
 & \multicolumn{2}{c}{Employment Counts} & & \multicolumn{2}{c}{$B$ Employment Share} & & \multicolumn{2}{c}{$F$ Employment Share} & & \multicolumn{2}{c}{wage, ($Z\_W3$)}  \\ \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}
        Statewide Distribution  & $B$ & $F$ & & Actual &Imputed* & &Actual &Imputed* & &Actual & Imputed**  \\ \midrule
        \textbf{Delaware} &  &  &  &  &  &  &  &  &  &  \\
\quad        Less than High School &  3,510  &  2,950  &  & 10.0\% & 10.1\% &  & 9.7\% &9.6\% &  &  \$6,100  &  \$6,180  \\
\quad        High School Graduate &  11,400  &  9,910  &  & 32.7\% & 27.7\% &  & 32.4\% &27.4\% &  &  \$7,590  &  \$7,590  \\
\quad        Some College or Associates Degree &  10,200  &  8,920  &  & 29.3\% & 30.6\% &  & 29.2\% &30.6\% &  &  \$8,950  &  \$9,110  \\
\quad        College Graduate or Greater &  9,760  &  8,770  &  & 28.0\% & 31.5\% &  & 28.7\% &32.4\% &  &  \$14,900  &  \$13,800  \\ \midrule
        \textbf{Illinois} &  &  &  &  &  &  &  &  &  &  \\
\quad         Less than High School &  51,500  &  45,100  &  & 8.29\% & 9.16\% &  & 8.07\%& 8.90\% &  &  \$6,390  &  \$6,390  \\
\quad         High School Graduate &  168,000  &  151,000  &  & 27.00\% & 28.40\% &  & 27.00\% &28.20\% &  &  \$7,520  &  \$7,730  \\
\quad         Some College or Associates Degree &  205,000  &  185,000  &  & 33.00\% & 31.40\% &  & 33.10\% &31.50\% &  &  \$8,880  &  \$9,530  \\
\quad         College Graduate or Greater &  197,000  &  178,000  &  & 31.80\% & 31.00\% &  & 31.90\% & 31.40\% &  &  \$15,700  &  \$15,100  \\  \midrule
        \textbf{New Jersey} &  &  &  &  &  &  &  &  &  &  \\
\quad         Less than High School &  31,500  &  27,300  &  & 9.14\% & 8.42\% &  & 8.93\% &8.12\% &  &  \$6,860  &  \$6,510  \\
\quad         High School Graduate &  95,800  &  85,100  &  & 27.80\% & 21.40\% &  & 27.80\% &21.10\% &  &  \$8,550  &  \$8,360  \\
\quad         Some College or Associates Degree &  93,100  &  82,600  &  & 27.00\% & 29.20\% &  & 27.00\% &29.20\% &  &  \$10,400  &  \$10,500  \\
\quad         College Graduate or Greater &  125,000  &  111,000  &  & 36.10\% & 41.00\% &  & 36.30\% &41.50\% &  &  \$17,700  &  \$16,400  \\
%    & & \multicolumn{4}{c}{Coefficient of Variation}  \\ \cmidrule{3-6}
\bottomrule
\end{tabular}

\footnotesize
\begin{tablenotes}
\item {\it Notes}: *Average share over ten implicates. **Average over ten implicates. Statistics computed for year 2000:2. $B$ denotes beginning-of-quarter employment, and $F$ denotes full-quarter employment.
\end{tablenotes}
\label{tab:stateqwi}
\end{threeparttable}
}%
\end{center}
\end{table}


==> tables/d_sample_state_sex.tex <==
\begin{table}[!htbp]
\begin{center}
\resizebox{\linewidth}{!}{
%\scalebox{0.70}{
    \begin{threeparttable}
        \caption{Comparison of QWI Variables for the Decennial Sample (D Sample) by Sex: Actual vs. Imputed Education}
    \begin{tabular}{llrrrrrrrrrrr} \toprule
        & & & & & & & & & & & \multicolumn{2}{c}{Average Full-quarter}  \\
        & & \multicolumn{2}{c}{Employment Counts} & & \multicolumn{2}{c}{$B$ Employment Share} & & \multicolumn{2}{c}{$F$ Employment Share} & & \multicolumn{2}{c}{wage, ($Z\_W3$)}  \\ \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
        \multicolumn{2}{l}{Statewide Distribution by Sex}  & $B$ & $F$ & & Actual &Imputed* & &Actual &Imputed* & &Actual & Imputed**  \\ \midrule
        \textbf{Delaware} &  &  &  &  &  &  &  &  &  &  &  &  \\
\quad        Female & Less than High School &  1,420  &  1,100  &  & 8.45\% & 8.59\% &  & 8.08\% & 8.04\% &  &  \$4,470  &  \$4,360  \\
         & High School Graduate &  5,450  &  4,750  &  & 32.50\% & 27.10\% &  & 32.40\% & 26.80\% &  &  \$5,810  &  \$5,610  \\
         & Some College or Associates Degree &  5,320  &  4,640  &  & 31.80\% & 32.40\% &  & 31.70\% & 32.40\% &  &  \$7,120  &  \$7,080  \\
        & College Graduate or Greater &  4,570  &  4,080  &  & 27.20\% & 31.90\% &  & 27.90\% & 32.70\% &  &  \$11,200  &  \$10,600  \\ \cmidrule{2-13}
\quad        Male & Less than High School &  2,100  &  1,780  &  & 11.50\% & 11.50\% &  & 11.10\% & 11.00\% &  &  \$7,190  &  \$7,400  \\
         & High School Graduate &  5,980  &  5,170  &  & 32.90\% & 28.30\% &  & 32.40\% & 28.00\% &  &  \$9,220  &  \$9,320  \\
         & Some College or Associates Degree &  4,910  &  4,300  &  & 27.00\% & 29.00\% &  & 27.00\% & 29.00\% &  &  \$10,900  &  \$11,200  \\
         & College Graduate or Greater &  5,300  &  4,700  &  & 28.60\% & 31.20\% &  & 29.50\% & 32.00\% &  &  \$18,100  &  \$16,900  \\ \midrule
        \textbf{Illinois} &  &  &  &  &  &  &  &  &  &  &  &  \\
\quad        Female & Less than High School &  22,900  &  20,000  &  & 7.46\% & 8.35\% &  & 7.28\% & 8.11\% &  &  \$4,500  &  \$4,510  \\
         & High School Graduate &  81,900  &  73,700  &  & 26.70\% & 28.90\% &  & 26.80\% & 28.80\% &  &  \$5,400  &  \$5,490  \\
         & Some College or Associates Degree &  107,000  &  95,900  &  & 34.90\% & 33.30\% &  & 35.00\% & 33.40\% &  &  \$6,600  &  \$6,960  \\
         & College Graduate or Greater &  95,000  &  84,900  &  & 31.00\% & 29.40\% &  & 30.90\% & 29.70\% &  &  \$10,900  &  \$10,800  \\ \cmidrule{2-13}
    \quad    Male & Less than High School &  28,700  &  25,200  &  & 9.10\% & 9.96\% &  & 8.84\% & 9.66\% &  &  \$7,880  &  \$7,900  \\
         & High School Graduate &  85,800  &  77,200  &  & 27.30\% & 28.00\% &  & 27.10\% & 27.70\% &  &  \$9,550  &  \$9,990  \\
         & Some College or Associates Degree &  97,900  &  88,900  &  & 31.10\% & 29.60\% &  & 31.20\% & 29.60\% &  &  \$11,300  &  \$12,300  \\
         & College Graduate or Greater &  102,000  &  93,400  &  & 32.50\% & 32.50\% &  & 32.80\% & 33.00\% &  &  \$20,100  &  \$18,900  \\ \midrule
        \textbf{New Jersey} &  &  &  &  &  &  &  &  &  &  &  &  \\
\quad        Female & Less than High School &  14,000  &  12,100  &  & 8.15\% & 7.80\% &  & 7.96\% & 7.52\% &  &  \$4,940  &  \$4,730  \\
         & High School Graduate &  49,300  &  43,900  &  & 28.70\% & 22.10\% &  & 28.80\% & 21.90\% &  &  \$6,450  &  \$6,070  \\
         & Some College or Associates Degree &  49,200  &  43,600  &  & 28.60\% & 31.10\% &  & 28.70\% & 31.10\% &  &  \$7,950  &  \$7,890  \\
         & College Graduate or Greater &  59,500  &  52,600  &  & 34.60\% & 39.00\% &  & 34.60\% & 39.50\% &  &  \$12,700  &  \$12,100  \\ \cmidrule{2-13}
\quad        Male & Less than High School &  17,500  &  15,200  &  & 10.10\% & 9.03\% &  & 9.90\% & 8.71\% &  &  \$8,390  &  \$8,040  \\
         & High School Graduate &  46,500  &  41,200  &  & 26.90\% & 20.60\% &  & 26.80\% & 20.30\% &  &  \$10,800  &  \$10,800  \\
         & Some College or Associates Degree &  43,900  &  38,900  &  & 25.40\% & 27.40\% &  & 25.30\% & 27.40\% &  &  \$13,100  &  \$13,600  \\
         & College Graduate or Greater &  65,100  &  58,400  &  & 37.60\% & 42.90\% &  & 38.00\% & 43.50\% &  &  \$22,100  &  \$20,200  \\
%    & & \multicolumn{4}{c}{Coefficient of Variation}  \\ \cmidrule{3-6}
\bottomrule
\end{tabular}

\footnotesize
\begin{tablenotes}
\item {\it Notes}: *Average share over ten implicates. **Average over ten implicates. Statistics computed for year 2000:2. $B$ denotes beginning-of-quarter employment, and $F$ denotes full-quarter employment.
\end{tablenotes}
\label{tab:stateqwisex}
\end{threeparttable}
}%
\end{center}
\end{table}


==> tables/emptotal_table.tex <==
\begin{landscape}
\begin{table}[htbp] 
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of Total Employment ($EmpTotal$) by Table and Count}
\begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 15}{c}{} \\ 

\multicolumn{ 1}{c}{Table and $EmpTotal$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Count} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Bounds Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule

%Panel A
\multicolumn{15}{c}{\textbf{A: Private}} \\ 
\input{\MyPathtv/tables/emptotal_table_paprivate.tex}

\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: 
\end{tablenotes}
\end{threeparttable}
}%
\label{tab:emptotal}
\end{table}
\end{landscape}



==> tables/emptotal_table_a.tex <==
Age x Gender & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  \\ 
\quad +1000 & 1.0000 &  46,480  & 80,832  &  & 8250.00 & 43.60\% &  & 0.0004 & 0.0011 & 0.0036 &  & 47 & 118 & 0.14\% \\ 
Race x Ethnicity & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad 10-99 & 0.0199 &  695  & 53  &  & 49.80 & 96.10\% &  & 0.0836 & 0.1409 & 0.2605 &  & 9 & 10 & 19.48\% \\ 
\quad 100-999 & 0.1306 &  4,553  & 452  &  & 411.00 & 95.30\% &  & 0.0242 & 0.0469 & 0.0935 &  & 9 & 28 & 6.49\% \\ 
\quad +1000 & 0.8495 &  29,612  & 13,614  &  & 5970.00 & 86.40\% &  & 0.0002 & 0.0044 & 0.0274 &  & 12 & 105 & 0.59\% \\ 
Gender x Education & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad +1000 & 1.0000 &  23,240  & 157,493  &  & 192000.00 & 96.60\% &  & 0.0013 & 0.0031 & 0.0086 &  & 9 & 606 & 0.43\% \\ 
Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0045 &  12,955  & 0  &  & 0.30 & 94.40\% & \multicolumn{1}{r}{} & (a) & (a) & (a) &  & 10 & 1 & (a) \\ 
\quad 1-2 & 0.0001 &  188  & 1  &  & 0.42 & 79.35\% &  & 0.1982 & 0.3913 & 0.9553 &  & 14 & 1 & 52.73\% \\ 
\quad 3-9 & 0.0158 &  45,741  & 7  &  & 0.50 & 0.00\% &  & 0.0614 & 0.1073 & 0.3800 &  & 9999 & 1 & 13.76\% \\ 
\quad 10-99 & 0.2603 &  753,131  & 46  &  & 4.82 & 15.40\% &  & 0.0242 & 0.0511 & 0.1619 &  & 380 & 3 & 6.56\% \\ 
\quad 100-999 & 0.4402 &  1,273,670  & 294  &  & 53.70 & 66.30\% &  & 0.0105 & 0.0235 & 0.0591 &  & 20 & 10 & 3.12\% \\ 
\quad +1000 & 0.2792 &  807,706  & 3,058  &  & 822.00 & 76.60\% &  & 0.0023 & 0.0081 & 0.0201 &  & 15 & 38 & 1.09\% \\ 
Age x Gender x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.2019 &  8,888,449  & 0  &  & 0.21 & 95.10\% & \multicolumn{1}{r}{} & (a) & (a) & (a) &  & 9 & 1 & (a) \\ 
\quad 1-2 & 0.0050 &  220,862  & 2  &  & 0.35 & 67.20\% &  & 0.1564 & 0.3066 & 0.7280 &  & 19 & 1 & 40.71\% \\ 
\quad 3-9 & 0.2171 &  9,557,988  & 5  &  & 0.81 & 61.50\% &  & 0.0885 & 0.1722 & 0.3887 &  & 23 & 1 & 22.73\% \\ 
\quad 10-99 & 0.3796 &  16,713,425  & 27  &  & 5.35 & 69.70\% &  & 0.0382 & 0.0815 & 0.1800 &  & 18 & 3 & 10.84\% \\ 
\quad 100-999 & 0.1622 &  7,142,409  & 225  &  & 55.20 & 75.40\% &  & 0.0142 & 0.0303 & 0.0618 &  & 15 & 10 & 4.06\% \\ 
\quad +1000 & 0.0343 &  1,511,324  & 1,972  &  & 502.00 & 75.70\% &  & 0.0041 & 0.0103 & 0.0201 &  & 15 & 30 & 1.38\% \\ 
Race x Ethnicity x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.5839 &  19,047,330  & 0  &  & 0.20 & 95.20\% & \multicolumn{1}{r}{} & (a) & (a) & (a) &  & 9 & 1 & (a) \\ 
\quad 1-2 & 0.0058 &  190,628  & 2  &  & 0.69 & 91.70\% &  & 0.2636 & 0.6229 & 0.9257 &  & 10 & 1 & 85.47\% \\ 
\quad 3-9 & 0.1330 &  4,339,494  & 5  &  & 2.35 & 88.90\% &  & 0.1325 & 0.3167 & 0.5963 &  & 11 & 2 & 43.18\% \\ 
\quad 10-99 & 0.1607 &  5,240,825  & 26  &  & 10.10 & 85.30\% &  & 0.0426 & 0.1162 & 0.2704 &  & 12 & 4 & 15.76\% \\ 
\quad 100-999 & 0.0830 &  2,707,617  & 249  &  & 75.90 & 79.90\% &  & 0.0137 & 0.0322 & 0.0745 &  & 14 & 12 & 4.33\% \\ 
\quad +1000 & 0.0336 &  1,094,612  & 2,586  &  & 766.00 & 79.20\% &  & 0.0031 & 0.0095 & 0.0212 &  & 14 & 37 & 1.28\% \\ 
Gender x Education x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0996 &  2,207,640  & 0  &  & 0.26 & 94.80\% & \multicolumn{1}{r}{} & (a) & (a) & (a) &  & 10 & 1 & (a) \\ 
\quad 1-2 & 0.0050 &  111,105  & 2  &  & 1.35 & 93.10\% &  & 0.4281 & 0.6538 & 0.9466 &  & 10 & 2 & 89.72\% \\ 
\quad 3-9 & 0.2024 &  4,484,091  & 5  &  & 3.99 & 92.70\% &  & 0.2395 & 0.3791 & 0.6106 &  & 10 & 3 & 52.03\% \\ 
\quad 10-99 & 0.4264 &  9,446,881  & 29  &  & 22.00 & 92.80\% &  & 0.0865 & 0.1624 & 0.2961 &  & 10 & 6 & 22.28\% \\ 
\quad 100-999 & 0.2119 &  4,695,684  & 235  &  & 190.00 & 93.10\% &  & 0.0292 & 0.0569 & 0.0967 &  & 10 & 19 & 7.81\% \\ 
\quad +1000 & 0.0546 &  1,209,869  & 2,089  &  & 1790.00 & 93.50\% &  & 0.0087 & 0.0193 & 0.0321 &  & 10 & 58 & 2.65\% \\ 


==> tables/emptotal_table_b.tex <==
Age x Gender & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  \\ 
\quad +1000 & 1.0000 &  46,480  & 91,515  &  & 8690.00 & 43.10\% &  & 0.0003 & 0.0010 & 0.0032 &  & 48 & 121 & 0.13\% \\ 
Race x Ethnicity & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad 10-99 & 0.0181 &  632  & 56  &  & 51.55 & 96.70\% &  & 0.0837 & 0.1403 & 0.2568 &  & 9 & 10 & 19.40\% \\ 
\quad 100-999 & 0.1223 &  4,263  & 443  &  & 415.00 & 95.60\% &  & 0.0265 & 0.0474 & 0.0932 &  & 9 & 28 & 6.56\% \\ 
\quad +1000 & 0.8596 &  29,965  & 14,956  &  & 6310.00 & 87.30\% &  & 0.0002 & 0.0041 & 0.0269 &  & 11 & 108 & 0.56\% \\ 
Gender x Education & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad +1000 & 1.0000 &  23,240  & 187,994  &  & 222000.00 & 96.80\% &  & 0.0012 & 0.0028 & 0.0079 &  & 9 & 652 & 0.39\% \\ 
Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  \\ 
\quad zero measured value, after rounding & 0.0026 &  8,225  & 0  &  & 0.31 & 94.90\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 10 & 1 & (a) \\ 
\quad 1-2 & 0.0000 &  134  & 1  &  & 0.39 & 80.10\% &  & 0.1664 & 0.3652 & 0.9434 &  & 14 & 1 & 49.21\% \\ 
\quad 3-9 & 0.0132 &  41,946  & 7  &  & 0.51 & 0.00\% &  & 0.0593 & 0.1075 & 0.3871 &  & 9999 & 1 & 13.78\% \\ 
\quad 10-99 & 0.2333 &  743,122  & 47  &  & 5.52 & 43.50\% &  & 0.0237 & 0.0537 & 0.1643 &  & 47 & 3 & 6.98\% \\ 
\quad 100-999 & 0.4539 &  1,445,825  & 307  &  & 57.90 & 70.80\% &  & 0.0101 & 0.0238 & 0.0593 &  & 18 & 10 & 3.17\% \\ 
\quad +1000 & 0.2971 &  946,236  & 2,989  &  & 774.00 & 77.10\% &  & 0.0023 & 0.0080 & 0.0199 &  & 15 & 37 & 1.08\% \\ 
Age x Gender x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.1672 &  7,973,123  & 0  &  & 0.21 & 95.20\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 1 & (a) \\ 
\quad 1-2 & 0.0049 &  234,460  & 2  &  & 0.38 & 72.70\% &  & 0.1527 & 0.3252 & 0.7382 &  & 17 & 1 & 43.36\% \\ 
\quad 3-9 & 0.2165 &  10,324,414  & 5  &  & 0.85 & 66.20\% &  & 0.0864 & 0.1754 & 0.3944 &  & 20 & 1 & 23.24\% \\ 
\quad 10-99 & 0.4014 &  19,140,564  & 27  &  & 5.33 & 71.40\% &  & 0.0367 & 0.0806 & 0.1803 &  & 17 & 3 & 10.75\% \\ 
\quad 100-999 & 0.1737 &  8,279,653  & 224  &  & 52.30 & 75.60\% &  & 0.0137 & 0.0294 & 0.0610 &  & 15 & 10 & 3.95\% \\ 
\quad +1000 & 0.0363 &  1,728,489  & 1,982  &  & 482.00 & 76.00\% &  & 0.0041 & 0.0101 & 0.0197 &  & 15 & 29 & 1.35\% \\ 
Race x Ethnicity x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.5635 &  19,553,448  & 0  &  & 0.20 & 95.50\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 1 & (a) \\ 
\quad 1-2 & 0.0062 &  216,005  & 2  &  & 0.70 & 92.10\% &  & 0.2688 & 0.6245 & 0.9354 &  & 10 & 1 & 85.69\% \\ 
\quad 3-9 & 0.1400 &  4,856,222  & 5  &  & 2.34 & 89.50\% &  & 0.1334 & 0.3159 & 0.5944 &  & 11 & 2 & 43.07\% \\ 
\quad 10-99 & 0.1653 &  5,735,093  & 26  &  & 10.10 & 86.20\% &  & 0.0431 & 0.1169 & 0.2692 &  & 12 & 4 & 15.85\% \\ 
\quad 100-999 & 0.0886 &  3,073,969  & 254  &  & 75.20 & 80.50\% &  & 0.0132 & 0.0317 & 0.0736 &  & 13 & 12 & 4.29\% \\ 
\quad +1000 & 0.0364 &  1,262,815  & 2,573  &  & 745.00 & 79.60\% &  & 0.0031 & 0.0093 & 0.0210 &  & 14 & 37 & 1.25\% \\ 
Gender x Education x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0737 &  1,787,333  & 0  &  & 0.26 & 95.10\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 1 & (a) \\ 
\quad 1-2 & 0.0044 &  106,593  & 2  &  & 1.38 & 93.40\% &  & 0.4290 & 0.6538 & 0.9513 &  & 10 & 2 & 89.72\% \\ 
\quad 3-9 & 0.1901 &  4,610,815  & 5  &  & 4.05 & 93.20\% &  & 0.2386 & 0.3783 & 0.6101 &  & 10 & 3 & 51.91\% \\ 
\quad 10-99 & 0.4433 &  10,755,591  & 29  &  & 22.50 & 93.20\% &  & 0.0853 & 0.1597 & 0.2946 &  & 10 & 7 & 21.91\% \\ 
\quad 100-999 & 0.2305 &  5,593,317  & 234  &  & 187.00 & 93.40\% &  & 0.0291 & 0.0566 & 0.0963 &  & 10 & 19 & 7.76\% \\ 
\quad +1000 & 0.0580 &  1,407,901  & 2,090  &  & 1770.00 & 93.70\% &  & 0.0084 & 0.0192 & 0.0318 &  & 10 & 58 & 2.63\% \\ 


==> tables/emptotal_table_private.tex <==
\begin{landscape}
\begin{table}[htbp]
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of Private Total Employment ($EmpTotal$) by Table and Count}
    \begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 1}{c}{Table and $EmpTotal$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Count} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Intervals Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
%
\multicolumn{15}{c}{\textbf{Private}} \\ 
\input{\MyPathtv/tables/emptotal_table_a.tex}
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Total employment is defined as all jobs held by a worker at the same establishment during the quarter. Statistics are computed across all state-year-quarters within a table. The ``Private" category of establishments includes only private establishments. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for total employment, please see their respective equations in the accompanying text:  Count \ref{eq:theb}, Total Variation \ref{eq:tvc}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.
    (a) Undefined value.
\end{tablenotes}
\label{tab:emptotprivate}
\end{threeparttable}
}%
\end{table}
\end{landscape}



==> tables/emptotal_table_total.tex <==
\begin{landscape}
\begin{table}[htbp]
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of All Total Employment ($EmpTotal$) by Table and Count}
    \begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 1}{c}{Table and $EmpTotal$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Count} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Intervals Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
%
        \multicolumn{15}{c}{\textbf{All (Private plus State and Local)}} \\ 
\input{\MyPathtv/tables/emptotal_table_b.tex}
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Total employment is defined as all jobs held by a worker at the same establishment during the quarter. Statistics are computed across all state-year-quarters within a table. The ``All" category of establishments includes private as well as state and local government but excludes federal employment. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for total employment, please see their respective equations in the accompanying text:  Count \ref{eq:theb}, Total Variation \ref{eq:tvc}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.
    (a) Undefined value.
\end{tablenotes}
\label{tab:emptotall}
\end{threeparttable}
}%
\end{table}
\end{landscape}



==> tables/fulemp_table.tex <==
\begin{landscape}
\begin{table}[htbp]
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of Full-Quarter Employment ($EmpS$) by Table and Count}
\begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 15}{c}{} \\ 

\multicolumn{ 1}{c}{Table and $EmpS$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Count} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Bounds Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
\multicolumn{15}{c}{\textbf{A: Private}} \\ 
Age x Gender &  \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} &  &  \\ 
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Total employment is defined as all jobs held by a worker at the same establishment during the quarter. Statistics are computed across all state-year-quarters within a table. The ``Private" category of establishments includes only private establishments. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for total employment, please see their respective equations in the accompanying text:  Count \ref{eq:theb}, Total Variation \ref{eq:tvc}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.
    (a) Undefined value.
\end{tablenotes}
\end{threeparttable}
}%
\label{tab:emps}
\end{table}
\end{landscape}



==> tables/fulemp_table_a.tex <==
Age x Gender & &  & & & & & & & & & & & &\\
\quad 100-999 & 0.0001 &  6  & 965  &  & 414.00 & 79.70\% &  & 0.0211 & 0.0211 & 0.0211 &  & 14 &27 & 2.84\% \\
\quad +1000 & 0.9999 &  44,938  & 50,251  &  & 3810.00 & 33.10\% &  & 0.0004 & 0.0012 & 0.0038 &  & 82&80 & 0.15\% \\
Race x Ethnicity & &  & & & & & & & & & & & &\\
\quad 3-9 & 0.0005 &  17  & 9  &  & 8.14 & 96.60\% &  & 0.1746 & 0.3394 & 0.4180 &  & 9&4 & 46.94\% \\
\quad 10-99 & 0.0351 &  1,184  & 46  &  & 32.70 & 95.10\% &  & 0.0747 & 0.1279 & 0.2935 &  & 9&8 & 17.69\% \\
\quad 100-999 & 0.1780 &  6,001  & 452  &  & 301.00 & 94.40\% &  & 0.0133 & 0.0420 & 0.0856 &  & 10&24 & 5.76\% \\
\quad +1000 & 0.7863 &  26,506  & 10,312  &  & 3290.00 & 80.60\% &  & 0.0002 & 0.0042 & 0.0239 &  & 13&77 & 0.56\% \\
Gender x Education & &  & & & & & & & & & & & &\\
\quad +1000 & 1.0000 &  22,472  & 115,661  &  & 114000.00 & 96.40\% &  & 0.0014 & 0.0031 & 0.0088 &  & 9&467 & 0.43\% \\
Industry x County & &  & & & & & & & & & & & &\\
\quad zero measured value, after rounding & 0.0142 &  40,036  & 0  &  & 0.28 & 95.60\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\
\quad 1-2 & 0.0002 &  505  & 2  &  & 0.19 & 0.00\% &  & 0.1308 & 0.2518 & 0.8485 &  & 9999&1 & 32.27\% \\
\quad 3-9 & 0.0327 &  92,014  & 7  &  & 0.40 & 0.00\% &  & 0.0571 & 0.1024 & 0.3636 &  & 9999&1 & 13.12\% \\
\quad 10-99 & 0.3147 &  886,839  & 43  &  & 4.21 & 23.50\% &  & 0.0231 & 0.0509 & 0.1608 &  & 162&3 & 6.55\% \\
\quad 100-999 & 0.4159 &  1,172,234  & 276  &  & 51.60 & 71.80\% &  & 0.0105 & 0.0241 & 0.0589 &  & 17&10 & 3.22\% \\
\quad +1000 & 0.2224 &  626,901  & 2,870  &  & 723.00 & 78.40\% &  & 0.0024 & 0.0081 & 0.0200 &  & 14&36 & 1.10\% \\
Age x Gender x Industry x County & &  & & & & & & & & & & & &\\
\quad zero measured value, after rounding & 0.2674 &  11,179,951  & 0  &  & 0.20 & 95.60\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\
\quad 1-2 & 0.0052 &  216,857  & 2  &  & 0.33 & 69.00\% &  & 0.1409 & 0.2958 & 0.7036 &  & 18&1 & 39.35\% \\
\quad 3-9 & 0.2274 &  9,509,759  & 5  &  & 0.71 & 62.50\% &  & 0.0808 & 0.1639 & 0.3791 &  & 23&1 & 21.63\% \\
\quad 10-99 & 0.3462 &  14,475,571  & 26  &  & 4.93 & 72.70\% &  & 0.0367 & 0.0805 & 0.1797 &  & 17&3 & 10.73\% \\
\quad 100-999 & 0.1295 &  5,413,281  & 221  &  & 50.70 & 77.40\% &  & 0.0134 & 0.0295 & 0.0611 &  & 15&10 & 3.96\% \\
\quad +1000 & 0.0243 &  1,017,595  & 1,896  &  & 429.00 & 76.50\% &  & 0.0041 & 0.0099 & 0.0194 &  & 15&28 & 1.33\% \\
Race x Ethnicity x Industry x  County & &  & & & & & & & & & & & &\\
\quad zero measured value, after rounding & 0.6503 &  20,835,268  & 0  &  & 0.19 & 95.80\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\
\quad 1-2 & 0.0049 &  157,195  & 2  &  & 0.65 & 92.20\% &  & 0.2579 & 0.6021 & 0.8874 &  & 10&1 & 82.62\% \\
\quad 3-9 & 0.1144 &  3,664,172  & 5  &  & 2.08 & 89.10\% &  & 0.1213 & 0.2990 & 0.5761 &  & 11&2 & 40.76\% \\
\quad 10-99 & 0.1366 &  4,375,170  & 26  &  & 8.75 & 84.90\% &  & 0.0385 & 0.1074 & 0.2582 &  & 12&4 & 14.56\% \\
\quad 100-999 & 0.0685 &  2,195,777  & 244  &  & 67.70 & 80.80\% &  & 0.0131 & 0.0306 & 0.0705 &  & 13&11 & 4.14\% \\
\quad +1000 & 0.0253 &  810,388  & 2,467  &  & 663.00 & 80.30\% &  & 0.0031 & 0.0093 & 0.0204 &  & 13&35 & 1.26\% \\
Gender x Education x Industry x County & &  & & & & & & & & & & & &\\
\quad zero measured value, after rounding & 0.1317 &  2,774,036  & 0  &  & 0.26 & 95.30\% &  & (a) & (a) & (a) &  & 9&1 & (a) \\
\quad 1-2 & 0.0059 &  124,663  & 2  &  & 1.32 & 93.80\% &  & 0.4278 & 0.6500 & 0.9368 &  & 10&2 & 89.19\% \\
\quad 3-9 & 0.2237 &  4,709,531  & 5  &  & 3.83 & 93.50\% &  & 0.2365 & 0.3766 & 0.6065 &  & 10&3 & 51.68\% \\
\quad 10-99 & 0.4122 &  8,679,900  & 27  &  & 20.60 & 93.60\% &  & 0.0860 & 0.1633 & 0.2954 &  & 10&6 & 22.40\% \\
\quad 100-999 & 0.1839 &  3,871,290  & 230  &  & 181.00 & 93.80\% &  & 0.0288 & 0.0564 & 0.0958 &  & 10&18 & 7.74\% \\
\quad +1000 & 0.0426 &  897,250  & 2,011  &  & 1640.00 & 94.20\% &  & 0.0086 & 0.0192 & 0.0315 &  & 10&56 & 2.64\% \\


==> tables/fulemp_table_b.tex <==
Age x Gender & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad 100-999 & 0.0001 &  3  & 961  &  & 402.00 & 79.30\% &  & 0.0209 & 0.0209 & 0.0209 &  & 14 & 27 & 2.81\% \\ 
\quad +1000 & 0.9999 &  44,941  & 56,533  &  & 4060.00 & 32.10\% &  & 0.0003 & 0.0011 & 0.0035 &  & 87 & 82 & 0.14\% \\ 
Race x Ethnicity & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0002 &  7  & 9  &  & 5.16 & 95.20\% &  & 0.2022 & 0.2589 & 0.4127 &  & 9 & 3 & 35.81\% \\ 
\quad 10-99 & 0.0323 &  1,088  & 48  &  & 35.15 & 95.70\% &  & 0.0737 & 0.1267 & 0.2891 &  & 9 & 8 & 17.53\% \\ 
\quad 100-999 & 0.1687 &  5,685  & 455  &  & 299.00 & 94.60\% &  & 0.0122 & 0.0420 & 0.0848 &  & 10 & 24 & 5.76\% \\ 
\quad +1000 & 0.7989 &  26,928  & 11,454  &  & 3550.00 & 81.90\% &  & 0.0001 & 0.0039 & 0.0235 &  & 13 & 80 & 0.52\% \\ 
Gender x Education & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad +1000 & 1.0000 &  22,472  & 143,578  &  & 134000.00 & 96.60\% &  & 0.0012 & 0.0029 & 0.0081 &  & 9 & 506 & 0.39\% \\ 
Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0085 &  26,395  & 0  &  & 0.27 & 95.50\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 1 & (a) \\ 
\quad 1-2 & 0.0001 &  445  & 2  &  & 0.20 & 0.00\% &  & 0.1178 & 0.2565 & 0.8139 &  & 9999 & 1 & 32.88\% \\ 
\quad 3-9 & 0.0273 &  84,593  & 7  &  & 0.41 & 0.00\% &  & 0.0557 & 0.1030 & 0.3814 &  & 9999 & 1 & 13.20\% \\ 
\quad 10-99 & 0.2858 &  884,129  & 44  &  & 5.06 & 51.60\% &  & 0.0228 & 0.0539 & 0.1654 &  & 33 & 3 & 7.05\% \\ 
\quad 100-999 & 0.4368 &  1,351,160  & 287  &  & 55.60 & 75.30\% &  & 0.0101 & 0.0245 & 0.0595 &  & 15 & 10 & 3.29\% \\ 
\quad +1000 & 0.2414 &  746,888  & 2,812  &  & 690.00 & 79.00\% &  & 0.0024 & 0.0081 & 0.0198 &  & 14 & 35 & 1.08\% \\ 
Age x Gender x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.2313 &  10,443,994  & 0  &  & 0.20 & 95.80\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 1 & (a) \\ 
\quad 1-2 & 0.0052 &  234,881  & 2  &  & 0.36 & 74.00\% &  & 0.1383 & 0.3166 & 0.7228 &  & 16 & 1 & 42.33\% \\ 
\quad 3-9 & 0.2281 &  10,301,188  & 5  &  & 0.75 & 67.40\% &  & 0.0789 & 0.1672 & 0.3849 &  & 19 & 1 & 22.20\% \\ 
\quad 10-99 & 0.3679 &  16,614,512  & 26  &  & 4.96 & 74.30\% &  & 0.0352 & 0.0799 & 0.1806 &  & 16 & 3 & 10.68\% \\ 
\quad 100-999 & 0.1410 &  6,367,152  & 220  &  & 48.10 & 77.50\% &  & 0.0130 & 0.0288 & 0.0605 &  & 15 & 9 & 3.86\% \\ 
\quad +1000 & 0.0265 &  1,197,767  & 1,914  &  & 417.00 & 76.90\% &  & 0.0040 & 0.0097 & 0.0191 &  & 15 & 27 & 1.30\% \\ 
Race x Ethnicity x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.6294 &  21,431,041  & 0  &  & 0.19 & 96.00\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 1 & (a) \\ 
\quad 1-2 & 0.0053 &  179,385  & 2  &  & 0.66 & 92.60\% &  & 0.2632 & 0.6042 & 0.8922 &  & 10 & 1 & 82.90\% \\ 
\quad 3-9 & 0.1210 &  4,119,278  & 5  &  & 2.08 & 89.70\% &  & 0.1232 & 0.2998 & 0.5754 &  & 11 & 2 & 40.88\% \\ 
\quad 10-99 & 0.1417 &  4,825,719  & 26  &  & 8.94 & 86.00\% &  & 0.0393 & 0.1088 & 0.2576 &  & 12 & 4 & 14.76\% \\ 
\quad 100-999 & 0.0746 &  2,541,058  & 249  &  & 67.80 & 81.50\% &  & 0.0126 & 0.0305 & 0.0701 &  & 13 & 11 & 4.11\% \\ 
\quad +1000 & 0.0281 &  955,663  & 2,460  &  & 637.00 & 80.80\% &  & 0.0031 & 0.0091 & 0.0202 &  & 13 & 34 & 1.22\% \\ 
Gender x Education x Industry x County & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ 
\quad zero measured value, after rounding & 0.0989 &  2,281,075  & 0  &  & 0.26 & 95.60\% & \multicolumn{1}{r}{} & (a) & (a) & (a) & \multicolumn{1}{r}{} & 9 & 1 & (a) \\ 
\quad 1-2 & 0.0053 &  121,268  & 2  &  & 1.37 & 94.10\% &  & 0.4295 & 0.6500 & 0.9421 &  & 10 & 2 & 89.19\% \\ 
\quad 3-9 & 0.2129 &  4,907,073  & 5  &  & 3.90 & 93.90\% &  & 0.2359 & 0.3763 & 0.6074 &  & 10 & 3 & 51.64\% \\ 
\quad 10-99 & 0.4341 &  10,007,726  & 28  &  & 21.10 & 93.90\% &  & 0.0849 & 0.1608 & 0.2945 &  & 10 & 6 & 22.06\% \\ 
\quad 100-999 & 0.2026 &  4,671,711  & 229  &  & 178.00 & 94.10\% &  & 0.0286 & 0.0562 & 0.0953 &  & 10 & 18 & 7.71\% \\ 
\quad +1000 & 0.0462 &  1,065,581  & 2,021  &  & 1620.00 & 94.30\% &  & 0.0087 & 0.0190 & 0.0312 &  & 10 & 55 & 2.60\% \\ 


==> tables/fulemp_table_private.tex <==
\begin{landscape}
\begin{table}[htbp]
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of Private Full-Quarter Employment ($EmpS$) by Table and Count}
\begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 15}{c}{} \\ 

\multicolumn{ 1}{c}{Table and $EmpS$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Count} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Intervals Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
\multicolumn{15}{c}{\textbf{Private}} \\ 
\input{\MyPathtv/tables/fulemp_table_a.tex}


\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Total employment is defined as all jobs held by a worker at the same establishment during the quarter. Statistics are computed across all state-year-quarters within a table. The ``Private" category of establishments includes only private establishments. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for total employment, please see their respective equations in the accompanying text:  Count \ref{eq:theb}, Total Variation \ref{eq:tvc}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.
    (a) Undefined value.
\end{tablenotes}
\label{tab:empspriv}
\end{threeparttable}
}%
\end{table}
\end{landscape}



==> tables/fulemp_table_total.tex <==
\begin{landscape}
\begin{table}[htbp]
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of All Full-Quarter Employment ($EmpS$) by Table and Count}
\begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 15}{c}{} \\ 

\multicolumn{ 1}{c}{Table and $EmpS$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Count} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Intervals Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
\multicolumn{15}{c}{\textbf{All (Private plus State and Local)}} \\ 
\input{\MyPathtv/tables/fulemp_table_b.tex}


\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Total employment is defined as all jobs held by a worker at the same establishment during the quarter. Statistics are computed across all state-year-quarters within a table. The ``All" category of establishments includes private as well as state and local government but excludes federal employment. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for total employment, please see their respective equations in the accompanying text:  Count \ref{eq:theb}, Total Variation \ref{eq:tvc}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.
    (a) Undefined value.
\end{tablenotes}
\label{tab:empsall}
\end{threeparttable}
}%
\end{table}
\end{landscape}



==> tables/imputes_education.tex <==
\begin{table}[htbp] 
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Distribution of ICF Categories across ACS Response Categories, Education}
    \begin{tabular}{llrrrr} \toprule 
\multicolumn{ 1}{c}{Distribution of catagories in ICF}& \multicolumn{ 1}{c}{90\% CI} & \multicolumn{ 1}{c}{$<$ High School} & \multicolumn{ 1}{c}{High School} &   \multicolumn{ 1}{c}{Some College} & \multicolumn{ 1}{c}{$\geq$ Bachelor} \\ \midrule 
 \textbf{Not in ACS} &  & & & & \\
\quad    Baseline: not imputed                                &  Upper & 13.8\% & 29.6\% & 30.5\% & 26.2\% \\ 
                                                              &  Mean & 13.7\% & 29.6\% & 30.5\% & 26.2\% \\ 
                                                              &  Lower & 13.7\% & 29.6\% & 30.5\% & 26.2\% \\ \midrule
 \textbf{ACS: Less than High School} &  & & & & \\
\quad    Impute: imputed, ACS is `$<$ High School'            &  Upper & 26.3\% & 33.8\% & 26.9\% & 14.3\% \\ 
                                                              &  Mean & 26.0\% & 33.5\% & 26.6\% & 14.0\% \\ 
                                                              &  Lower & 25.6\% & 33.1\% & 26.4\% & 13.6\% \\ 
\quad    Target: not imputed, ACS is `$<$ High School'        &  Upper & 80.8\% & 15.0\% & 4.2\% & 1.1\% \\ 
                                                              &  Mean & 80.4\% & 14.7\% & 4.0\% & 1.0\% \\ 
                                                              &  Lower & 80.0\% & 14.3\% & 3.8\% & 0.9\% \\ \midrule
 \textbf{ACS: High School} &  & & & & \\
\quad    Impute: imputed, ACS is `High School'                &  Upper & 14.8\% & 35.6\% & 31.6\% & 18.8\% \\ 
                                                              &  Mean & 14.6\% & 35.4\% & 31.4\% & 18.6\% \\ 
                                                              &  Lower & 14.5\% & 35.1\% & 31.2\% & 18.4\% \\ 
\quad    Target: not imputed, ACS is `High School'            &  Upper & 6.5\% & 81.5\% & 12.0\% & 0.9\% \\ 
                                                              &  Mean & 6.3\% & 81.2\% & 11.7\% & 0.8\% \\ 
                                                              &  Lower & 6.1\% & 80.8\% & 11.4\% & 0.7\% \\ \midrule
 \textbf{ACS: Some College} &  & & & & \\                       
\quad    Impute: imputed, ACS is `Some College'               &  Upper & 11.0\% & 29.9\% & 33.5\% & 26.4\% \\ 
                                                              &  Mean & 10.8\% & 29.7\% & 33.3\% & 26.2\% \\ 
                                                              &  Lower & 10.7\% & 29.5\% & 33.1\% & 25.9\% \\ 
\quad    Target: not imputed, ACS is `Some College'           &  Upper & 1.4\% & 11.3\% & 85.2\% & 3.0\% \\ 
                                                              &  Mean & 1.3\% & 11.0\% & 84.8\% & 2.9\% \\ 
                                                              &  Lower & 1.2\% & 10.7\% & 84.5\% & 2.7\% \\ \midrule
\textbf{ACS: $\geq$ Bachelors} &  & & & & \\
\quad    Impute: imputed, ACS is `$\geq$ Bachelors'           &  Upper & 6.1\% & 19.0\% & 28.6\% & 47.2\% \\ 
                                                              &  Mean & 6.0\% & 18.8\% & 28.4\% & 46.9\% \\ 
                                                              &  Lower & 5.8\% & 18.6\% & 28.1\% & 46.6\% \\ 
\quad    Target: not imputed, ACS is `$\geq$ Bachelors        &  Upper & 0.3\% & 0.9\% & 4.8\% & 94.6\% \\ 
                                                              &  Mean & 0.2\% & 0.8\% & 4.6\% & 94.3\% \\ 
                                                              &  Lower & 0.2\% & 0.7\% & 4.4\% & 94.1\% \\ 
                                                      
\bottomrule    
\end{tabular}
%}%
\footnotesize
\begin{tablenotes}
\item {\it Notes}: 90\% CI are 90\% confidence intervals of the mean. Major row heading is the value of the ACS variable. Minor row heading is the value of the ICF variable. Major row header ``Not in ACS'' denotes records that did not match to the ACS.
\end{tablenotes}
\label{tab:imped}
\end{threeparttable}
}%
\end{table}


==> tables/imputes_ethnicity.tex <==
\begin{table}[htbp] 
%\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Distribution of ICF Categories across ACS Response Categories, Ethnicity}
    \begin{tabular}{llrr} \toprule 
\multicolumn{ 1}{c}{Distribution of catagories in ICF}& \multicolumn{ 1}{c}{90\% CI} & \multicolumn{ 1}{c}{Not Hispanic} & \multicolumn{ 1}{c}{Hispanic} \\ \midrule 
 \textbf{Not in ACS} &  & &  \\
        \quad    Baseline: not imputed    &   Upper & 90.7\% & 9.3\% \\ 
                                          &   Mean & 90.7\% & 9.3\% \\ 
                                          &   Lower & 90.7\% & 9.3\% \\ \midrule
 \textbf{ACS: Not Hispanic} &  & &  \\
\quad    Impute: imputed, ACS is `Not Hispanic'         &       Upper & 94.7\% & 6.0\% \\ 
                                                        &       Mean & 94.4\% & 5.6\% \\ 
                                                        &       Lower & 94.0\% & 5.3\% \\ 
 \quad    Target: not imputed, ACS is `Not Hispanic'    &       Upper & 99.7\% & 0.4\% \\ 
                                                        &       Mean & 99.6\% & 0.4\% \\ 
                                                        &       Lower & 99.6\% & 0.3\% \\ \midrule
 \textbf{ACS: Hispanic} &  & &  \\
 \quad    Impute: imputed, ACS is `Hispanic'            &          Upper & 21.7\% & 81.7\% \\ 
                                                        &          Mean & 20.0\% & 80.0\% \\ 
                                                        &          Lower & 18.3\% & 78.3\% \\ 
 \quad    Target: not imputed, ACS is `Hispanic'        &          Upper & 5.5\% & 95.0\% \\ 
                                                        &          Mean & 5.2\% & 94.8\% \\ 
                                                        &          Lower & 5.0\% & 94.5\% \\ 
                                                     
\bottomrule    
\end{tabular}
%}%
\footnotesize
\begin{tablenotes}
\item {\it Notes}: 90\% CI are 90\% confidence intervals of the mean. Major row heading is the value of the ACS variable. Minor row heading is the value of the ICF variable. Major row header ``Not in ACS'' denotes records that did not match to the ACS.
\end{tablenotes}
\label{tab:impeth}
\end{threeparttable}
%}%
\end{table}


==> tables/imputes_race.tex <==
\begin{table}[htbp] 
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Distribution of ICF Categories across ACS Response Categories, Race}
    \begin{tabular}{llrrrrrr} \toprule 
        \multicolumn{ 1}{c}{Distribution of catagories in ICF}& \multicolumn{ 1}{c}{90\% CI} & \multicolumn{ 1}{c}{White} & \multicolumn{ 1}{c}{Black} &   \multicolumn{ 1}{c}{Native Amer.} & \multicolumn{ 1}{c}{$\geq$ Asian} &   \multicolumn{ 1}{c}{Hawaiian \& PI} & \multicolumn{ 1}{c}{$\geq$ Two or More}\\ \midrule 
\textbf{Not in ACS} &  & & & & & & \\
        \quad    Baseline: not imputed                     & Upper & 83.1\% & 11.1\% & 0.8\% & 3.9\% & 0.1\% & 1.0\% \\ 
                                                           & Mean & 83.1\% & 11.1\% & 0.8\% & 3.9\% & 0.1\% & 1.0\% \\ 
                                                           & Lower & 83.1\% & 11.1\% & 0.8\% & 3.9\% & 0.1\% & 1.0\% \\ \midrule
\textbf{ACS: White} &  & & & &  & & \\
\quad    Impute: imputed, ACS is `White'                   & Upper & 94.8\% & 2.0\% & 1.2\% & 1.0\% & 0.4\% & 1.5\% \\ 
                                                           & Mean & 94.5\% & 1.9\% & 1.1\% & 0.9\% & 0.3\% & 1.4\% \\ 
                                                           & Lower & 94.2\% & 1.7\% & 0.9\% & 0.7\% & 0.3\% & 1.2\% \\ 
\quad    Target: not imputed, ACS is `White'               & Upper & 99.3\% & 0.2\% & 0.1\% & 0.1\% & 0.0\% & 0.4\% \\ 
                                                           & Mean & 99.3\% & 0.2\% & 0.1\% & 0.1\% & 0.0\% & 0.3\% \\ 
                                                           & Lower & 99.2\% & 0.2\% & 0.1\% & 0.1\% & 0.0\% & 0.3\% \\ \midrule 
 \textbf{ACS: Black} &  & & & & \\
\quad    Impute: imputed, ACS is `Black'                   & Upper & 7.3\% & 90.8\% & 1.0\% & 1.2\% & 0.6\% & 3.0\% \\ 
                                                           & Mean & 6.3\% & 89.5\% & 0.6\% & 0.8\% & 0.4\% & 2.4\% \\ 
                                                           & Lower & 5.3\% & 88.3\% & 0.3\% & 0.4\% & 0.1\% & 1.7\% \\ 
\quad    Target: not imputed, ACS is `Black'               & Upper & 2.4\% & 96.9\% & 0.2\% & 0.2\% & 0.0\% & 0.9\% \\ 
                                                           & Mean & 2.2\% & 96.7\% & 0.1\% & 0.1\% & 0.0\% & 0.8\% \\ 
                                                           & Lower & 2.0\% & 96.5\% & 0.1\% & 0.1\% & 0.0\% & 0.7\% \\\midrule 
 \textbf{ACS: Native American} &  & & & & \\
\quad    Impute: imputed, ACS is `Native Amer.'            & Upper & 52.9\% & 8.6\% & 46.5\% & 7.6\% & 1.6\% & 8.5\% \\ 
                                                           & Mean & 45.5\% & 5.3\% & 39.2\% & 4.5\% & 0.5\% & 5.1\% \\ 
                                                           & Lower & 38.0\% & 2.0\% & 31.8\% & 1.4\% & 0.0\% & 1.6\% \\ 
\quad    Target: not imputed, ACS is `Native Amer.'        & Upper & 18.1\% & 2.5\% & 73.4\% & 2.1\% & 0.3\% & 10.2\% \\ 
                                                           & Mean & 16.4\% & 1.9\% & 71.3\% & 1.5\% & 0.1\% & 8.9\% \\ 
                                                           & Lower & 14.7\% & 1.2\% & 69.2\% & 0.9\% & 0.0\% & 7.6\% \\ \midrule 
 \textbf{ACS: Asian} &  & & & & \\
\quad    Impute: imputed, ACS is `Asian'                   & Upper & 10.7\% & 3.0\% & 1.5\% & 86.2\% & 1.6\% & 5.0\% \\ 
                                                           & Mean & 8.8\% & 2.0\% & 0.8\% & 83.7\% & 0.9\% & 3.7\% \\ 
                                                           & Lower & 6.9\% & 1.1\% & 0.2\% & 81.3\% & 0.3\% & 2.4\% \\ 
\quad    Target: not imputed, ACS is `Asian'               & Upper & 2.6\% & 0.6\% & 0.2\% & 94.9\% & 0.2\% & 2.8\% \\ 
                                                           & Mean & 2.3\% & 0.5\% & 0.2\% & 94.5\% & 0.1\% & 2.5\% \\ 
                                                           & Lower & 2.0\% & 0.3\% & 0.1\% & 94.0\% & 0.1\% & 2.1\% \\ \midrule 
        \textbf{ACS: Hawaiian \& PI} &  & & & & \\
\quad    Impute: imputed, ACS is `Hawaiian \& PI'             & Upper & 53.1\% & 17.5\% & 6.3\% & 54.7\% & 18.5\% & 23.3\% \\ 
                                                              & Mean & 35.1\% & 7.6\% & 1.5\% & 36.5\% & 8.1\% & 11.3\% \\ 
                                                              & Lower & 17.1\% & 0.0\% & 0.0\% & 18.3\% & 0.0\% & 0.0\% \\ 
\quad    Target: not imputed, ACS is `Hawaiian \& PI'         & Upper & 13.7\% & 6.3\% & 1.4\% & 19.9\% & 53.0\% & 27.8\% \\ 
                                                              & Mean & 10.1\% & 4.0\% & 0.5\% & 15.6\% & 47.0\% & 22.8\% \\ 
                                                              & Lower & 6.5\% & 1.6\% & 0.0\% & 11.3\% & 41.1\% & 17.8\% \\ \midrule
 \textbf{ACS: Two or More} &  & & & & \\
\quad    Impute: imputed, ACS is `Two or More'                & Upper & 89.4\% & 7.0\% & 3.3\% & 3.5\% & 1.0\% & 2.5\% \\ 
                                                              & Mean & 87.3\% & 5.6\% & 2.3\% & 2.5\% & 0.6\% & 1.7\% \\ 
                                                              & Lower & 85.2\% & 4.1\% & 1.4\% & 1.6\% & 0.1\% & 0.9\% \\ 
\quad    Target: not imputed, ACS is `Two or More'            & Upper & 85.1\% & 6.4\% & 2.9\% & 4.6\% & 0.4\% & 2.9\% \\ 
                                                              & Mean & 84.4\% & 5.9\% & 2.6\% & 4.2\% & 0.3\% & 2.6\% \\ 
                                                              & Lower & 83.6\% & 5.5\% & 2.2\% & 3.9\% & 0.2\% & 2.3\% \\ \midrule
\textbf{ACS: Some Other} &  & & & & \\
\quad    Impute: imputed, ACS is `Some Other'                 & Upper & 64.8\% & 19.5\% & 5.3\% & 15.0\% & 2.7\% & 6.4\% \\ 
                                                              & Mean & 60.9\% & 16.5\% & 3.8\% & 12.4\% & 1.7\% & 4.7\% \\ 
                                                              & Lower & 57.0\% & 13.6\% & 2.3\% & 9.8\% & 0.6\% & 3.0\% \\ 
\quad    Target: not imputed, ACS is `Some Other'             & Upper & 41.0\% & 10.1\% & 8.0\% & 7.3\% & 2.8\% & 35.6\% \\ 
                                                              & Mean & 39.8\% & 9.4\% & 7.3\% & 6.7\% & 2.4\% & 34.5\% \\ 
                                                              & Lower & 38.6\% & 8.6\% & 6.7\% & 6.1\% & 2.0\% & 33.3\% \\ 

\bottomrule    
\end{tabular}
%}%
\footnotesize
\begin{tablenotes}
\item {\it Notes}: 90\% CI are 90\% confidence intervals of the mean. Major row heading is the value of the ACS variable. Minor row heading is the value of the ICF variable. Major row header ``Not in ACS'' denotes records that did not match to the ACS.
\end{tablenotes}
\label{tab:imprace}
\end{threeparttable}
}%
\end{table}


==> tables/payroll_table.tex <==
\begin{landscape}
\begin{table}[htbp]
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of Total Payroll ($Payroll$) by Table and Count}
\begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 15}{c}{} \\ 

\multicolumn{ 1}{c}{Table and $EmpTotal$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Count} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Bounds Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
\multicolumn{15}{c}{\textbf{Private}} \\ 

\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Total Payroll is defined only over total employment. It is calculated by summing the earnings for the reference quarter for total employment.  See the table on total employment for the relevent counts. Statistics are computed across all state-year-quarters within a table. The ``All" category of establishments includes private as well as state, and local government but excludes federal employment. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for beginning of quarter employment, please see their respective equations in the accompanying text:  Total payroll \ref{eq:w1pub}, Total Variation \ref{eq:tvw1}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.  
 (a) Undefined value.
\end{tablenotes}
\end{threeparttable}
}%
\label{tab:payroll}
\end{table}
\end{landscape}



==> tables/payroll_table_a.tex <==
Age x Gender & &  & & & & & & & & & & & &\\
\quad +1000 & 1.0000 &  46,480  & 375,627,224.50  &  & 3.96E+11 & 29.50\% &  & 0.0005 & 0.0016 & 0.0083 &  & 104& 811,617.46  & 0.21\% \\
Race x Ethnicity & &  & & & & & & & & & & & &\\
\quad 10-99 & 0.0199 &  695  & 233,792.00  &  & 2.29E+09 & 97.30\% &  & 0.1187 & 0.2083 & 0.4509 &  & 9& 66,183.38  & 28.80\% \\
\quad 100-999 & 0.1306 &  4,553  & 2,166,851.00  &  & 1.85E+10 & 96.10\% &  & 0.0334 & 0.0678 & 0.1493 &  & 9& 188,112.25  & 9.38\% \\
\quad +1000 & 0.8495 &  29,612  & 71,561,892.50  &  & 4.67E+11 & 82.40\% &  & 0.0005 & 0.0070 & 0.0479 &  & 13& 922,671.93  & 0.94\% \\
Gender x Education & &  & & & & & & & & & & & &\\
\quad +1000 & 1.0000 &  23,240  & 1,122,441,816.50  &  & 2.05E+13 & 96.10\% &  & 0.0018 & 0.0042 & 0.0117 &  & 9& 6,261,928.94  & 0.57\% \\
\quad Industry x County & &  & & & & & & & & & & & &\\
\quad zero measured value, after rounding & 0.0040 &  12,955  & 0.00  &  & 9.45E+06 & 99.80\% &  & 0.0392 & 0.4429 & 1.0808 &  & 9& 4,251.55  & 61.25\% \\
\quad 1-2 & 0.1144 &  373,579  & 39,363.00  &  & 8.17E+06 & 0.00\% &  & 0.0000 & 0.0671 & 0.5900 &  & 9999& 3,663.33  & 8.60\% \\
\quad 3-9 & 0.0140 &  45,741  & 28,035.00  &  & 5.56E+06 & 0.00\% &  & 0.0302 & 0.0834 & 0.5458 &  & 9999& 3,022.05  & 10.68\% \\
\quad 10-99 & 0.2305 &  753,131  & 214,551.00  &  & 1.23E+08 & 9.57\% &  & 0.0198 & 0.0536 & 0.2327 &  & 984& 14,222.64  & 6.88\% \\
\quad 100-999 & 0.3899 &  1,273,670  & 1,568,970.00  &  & 2.55E+09 & 76.50\% &  & 0.0108 & 0.0307 & 0.0905 &  & 15& 67,697.26  & 4.12\% \\
\quad +1000 & 0.2473 &  807,706  & 19,017,146.50  &  & 6.38E+10 & 80.70\% &  & 0.0035 & 0.0118 & 0.0329 &  & 13& 341,035.20  & 1.59\% \\
Age x Gender x Industry x County & &  & & & & & & & & & & & &\\
\quad zero measured value, after rounding & 0.1701 &  8,888,449  & 0.00  &  & 6.05E+05 & 100.00\% &  & 0.0000 & 0.2197 & 1.3084 &  & 9& 1,075.74  & 30.39\% \\
\quad 1-2 & 0.1618 &  8,454,917  & 4,523.00  &  & 3.34E+05 & 12.30\% &  & 0.0000 & 0.1107 & 0.8974 &  & 598& 741.46  & 14.20\% \\
\quad 3-9 & 0.1829 &  9,557,988  & 17,743.00  &  & 8.87E+06 & 83.20\% &  & 0.0453 & 0.1636 & 0.6023 &  & 13& 4,021.15  & 22.08\% \\
\quad 10-99 & 0.3198 &  16,713,425  & 113,931.00  &  & 1.16E+08 & 85.80\% &  & 0.0327 & 0.0939 & 0.2689 &  & 12& 14,606.91  & 12.73\% \\
\quad 100-999 & 0.1367 &  7,142,409  & 1,166,690.00  &  & 2.00E+09 & 87.20\% &  & 0.0144 & 0.0384 & 0.0942 &  & 11& 60,974.46  & 5.23\% \\
\quad +1000 & 0.0289 &  1,511,324  & 14,164,728.00  &  & 3.60E+10 & 84.30\% &  & 0.0049 & 0.0135 & 0.0327 &  & 12& 257,324.15  & 1.83\% \\
Race x Ethnicity x Industry x  County & &  & & & & & & & & & & & &\\
\quad zero measured value, after rounding & 0.4859 &  19,047,330  & 0.00  &  & 3.28E+06 & 100.00\% &  & 0.0115 & 0.4685 & 1.5608 &  & 9& 2,504.77  & 64.80\% \\
\quad 1-2 & 0.1727 &  6,771,506  & 4,934.00  &  & 6.96E+06 & 98.50\% &  & 0.0745 & 0.5842 & 1.2527 &  & 9& 3,648.68  & 80.80\% \\
\quad 3-9 & 0.1107 &  4,339,494  & 20,418.00  &  & 6.02E+07 & 96.70\% &  & 0.1040 & 0.4024 & 0.8577 &  & 9& 10,730.73  & 55.65\% \\
\quad 10-99 & 0.1337 &  5,240,825  & 125,020.00  &  & 3.38E+08 & 93.50\% &  & 0.0423 & 0.1488 & 0.3976 &  & 10& 25,227.29  & 20.42\% \\
\quad 100-999 & 0.0691 &  2,707,617  & 1,330,383.00  &  & 3.50E+09 & 88.60\% &  & 0.0153 & 0.0433 & 0.1145 &  & 11& 80,661.63  & 5.90\% \\
\quad +1000 & 0.0279 &  1,094,612  & 16,504,365.00  &  & 5.75E+10 & 84.60\% &  & 0.0044 & 0.0135 & 0.0349 &  & 12& 325,209.49  & 1.83\% \\
Gender x Education x Industry x County & &  & & & & & & & & & & & &\\
\quad zero measured value, after rounding & 0.0845 &  2,207,640  & 153.00  &  & 2.35E+05 & 99.50\% &  & 0.0000 & 0.1886 & 2.1637 &  & 9& 670.45  & 26.08\% \\
\quad 1-2 & 0.1565 &  4,089,395  & 6,804.00  &  & 1.91E+07 & 98.80\% &  & 0.3127 & 0.6056 & 1.1470 &  & 9& 6,044.33  & 83.76\% \\
\quad 3-9 & 0.1716 &  4,484,091  & 25,232.00  &  & 1.38E+08 & 97.90\% &  & 0.2627 & 0.4790 & 0.8323 &  & 9& 16,246.91  & 66.24\% \\
\quad 10-99 & 0.3615 &  9,446,881  & 160,107.00  &  & 1.10E+09 & 97.20\% &  & 0.1026 & 0.2084 & 0.4189 &  & 9& 45,869.87  & 28.83\% \\
\quad 100-999 & 0.1797 &  4,695,684  & 1,522,171.00  &  & 1.37E+10 & 96.90\% &  & 0.0367 & 0.0763 & 0.1454 &  & 9& 161,879.36  & 10.55\% \\
\quad +1000 & 0.0463 &  1,209,869  & 17,075,678.00  &  & 2.34E+11 & 96.40\% &  & 0.0118 & 0.0277 & 0.0559 &  & 9& 669,020.05  & 3.83\% \\


==> tables/payroll_table_b.tex <==
Age x Gender & &  & & & & & & & & & & & &\\ 
\quad +1000 & 1.0000 &  46,480  & 431,844,381.50 &  & 4.06E+11 & 30.00\% &  & 0.0004 & 0.0014 & 0.0078 &  & 99 &  822,066.74  & 0.18\% \\ 
Race x Ethnicity & &  & & & & & & & & & & & &\\ 
\quad 10-99 & 0.0181 &  632  & 248,224.00 &  & 2.23E+09 & 97.70\% &  & 0.1058 & 0.2015 & 0.4318 &  & 9 &  65,310.59  & 27.87\% \\ 
\quad 100-999 & 0.1223 &  4,263  & 2,153,721.00 &  & 1.82E+10 & 96.30\% &  & 0.0348 & 0.0672 & 0.1469 &  & 9 &  186,580.78  & 9.29\% \\ 
\quad +1000 & 0.8596 &  29,965  & 80,813,010.00 &  & 4.83E+11 & 83.80\% &  & 0.0004 & 0.0063 & 0.0449 &  & 12 &  942,546.65  & 0.85\% \\ 
Gender x Education & &  & & & & & & & & & & & &\\ 
\quad +1000 & 1.0000 &  23,240  & 1,344,933,652.50 &  & 2.35E+13 & 96.60\% &  & 0.0016 & 0.0038 & 0.0110 &  & 9 &  6,704,480.56  & 0.53\% \\ 
\quad Industry x County & &  & & & & & & & & & & & &\\ 
\quad zero measured value, after rounding & 0.0024 &  8,225  & 0.00 &  & 9.59E+06 & 99.80\% &  & 0.0529 & 0.4142 & 1.2418 &  & 9 &  4,282.93  & 57.28\% \\ 
\quad 1-2 & 0.0886 &  309,518  & 47,962.00 &  & 1.43E+07 & 0.00\% &  & 0.0000 & 0.0656 & 0.5918 &  & 9999 &  4,846.55  & 8.41\% \\ 
\quad 3-9 & 0.0120 &  41,946  & 27,741.50 &  & 6.22E+06 & 0.00\% &  & 0.0299 & 0.0854 & 0.5657 &  & 9999 &  3,196.39  & 10.95\% \\ 
\quad 10-99 & 0.2126 &  743,122  & 223,252.00 &  & 1.72E+08 & 56.10\% &  & 0.0193 & 0.0590 & 0.2425 &  & 28 &  17,213.63  & 7.74\% \\ 
\quad 100-999 & 0.4137 &  1,445,825  & 1,652,146.00 &  & 2.85E+09 & 83.00\% &  & 0.0100 & 0.0314 & 0.0903 &  & 13 &  72,079.42  & 4.25\% \\ 
\quad +1000 & 0.2708 &  946,236  & 19,043,488.50 &  & 5.83E+10 & 82.90\% &  & 0.0033 & 0.0111 & 0.0315 &  & 13 &  326,004.16  & 1.49\% \\ 
Age x Gender x Industry x County & &  & & & & & & & & & & & &\\ 
\quad zero measured value, after rounding & 0.1426 &  7,973,123  & 0.00 &  & 5.66E+05 & 99.90\% &  & 0.0000 & 0.3606 & 5.6209 &  & 9 &  1,040.49  & 49.87\% \\ 
\quad 1-2 & 0.1515 &  8,471,709  & 4,432.00 &  & 4.34E+05 & 52.60\% &  & 0.0000 & 0.1250 & 0.9335 &  & 32 &  862.07  & 16.35\% \\ 
\quad 3-9 & 0.1846 &  10,324,414  & 17,514.00 &  & 1.00E+07 & 87.70\% &  & 0.0458 & 0.1819 & 0.6249 &  & 11 &  4,311.55  & 24.80\% \\ 
\quad 10-99 & 0.3423 &  19,140,564  & 116,677.00 &  & 1.23E+08 & 87.70\% &  & 0.0309 & 0.0949 & 0.2717 &  & 11 &  15,121.17  & 12.94\% \\ 
\quad 100-999 & 0.1481 &  8,279,653  & 1,215,134.00 &  & 2.00E+09 & 87.90\% &  & 0.0131 & 0.0368 & 0.0921 &  & 11 &  60,974.46  & 5.01\% \\ 
\quad +1000 & 0.0309 &  1,728,489  & 14,814,716.00 &  & 3.50E+10 & 85.30\% &  & 0.0045 & 0.0126 & 0.0311 &  & 12 &  253,725.03  & 1.71\% \\ 
Race x Ethnicity x Industry x County & &  & & & & & & & & & & & &\\ 
\quad zero measured value, after rounding & 0.4663 &  19,553,448  & 0.00 &  & 3.51E+06 & 100.00\% &  & 0.0387 & 0.4623 & 2.8196 &  & 9 &  2,591.10  & 63.93\% \\ 
\quad 1-2 & 0.1778 &  7,456,341  & 5,093.00 &  & 8.21E+06 & 98.60\% &  & 0.0824 & 0.6106 & 1.2213 &  & 9 &  3,962.81  & 84.45\% \\ 
\quad 3-9 & 0.1158 &  4,856,222  & 21,430.50 &  & 6.60E+07 & 97.00\% &  & 0.1083 & 0.4033 & 0.8508 &  & 9 &  11,235.78  & 55.77\% \\ 
\quad 10-99 & 0.1368 &  5,735,093  & 129,598.00 &  & 3.71E+08 & 94.20\% &  & 0.0441 & 0.1494 & 0.3933 &  & 10 &  26,430.12  & 20.49\% \\ 
\quad 100-999 & 0.0733 &  3,073,969  & 1,398,948.00 &  & 3.58E+09 & 89.90\% &  & 0.0141 & 0.0421 & 0.1103 &  & 11 &  81,578.26  & 5.74\% \\ 
\quad +1000 & 0.0301 &  1,262,815  & 16,919,665.00 &  & 5.45E+10 & 86.00\% &  & 0.0039 & 0.0127 & 0.0339 &  & 12 &  316,612.12  & 1.72\% \\ 
Gender x Education x Industry x County & &  & & & & & & & & & & & &\\ 
\quad zero measured value, after rounding & 0.0639 &  1,787,333  & 240.00 &  & 2.85E+05 & 99.60\% &  & 0.0000 & 0.2135 & 1.9833 &  & 9 &  738.34  & 29.53\% \\ 
\quad 1-2 & 0.1360 &  3,803,163  & 7,036.00 &  & 2.13E+07 & 98.90\% &  & 0.3025 & 0.6337 & 1.2283 &  & 9 &  6,382.94  & 87.65\% \\ 
\quad 3-9 & 0.1649 &  4,610,815  & 25,593.00 &  & 1.41E+08 & 98.10\% &  & 0.2569 & 0.4754 & 0.8347 &  & 9 &  16,422.56  & 65.75\% \\ 
\quad 10-99 & 0.3847 &  10,755,591  & 165,697.00 &  & 1.13E+09 & 97.50\% &  & 0.1005 & 0.2040 & 0.4132 &  & 9 &  46,491.16  & 28.21\% \\ 
\quad 100-999 & 0.2001 &  5,593,317  & 1,541,163.00 &  & 1.33E+10 & 97.30\% &  & 0.0356 & 0.0740 & 0.1405 &  & 9 &  159,498.65  & 10.23\% \\ 
\quad +1000 & 0.0504 &  1,407,901  & 17,357,576.00 &  & 2.23E+11 & 96.80\% &  & 0.0112 & 0.0266 & 0.0535 &  & 9 &  653,105.94  & 3.67\% \\ 


==> tables/payroll_table_private.tex <==
\begin{landscape}
\begin{table}[htbp]
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of Private Total Payroll ($Payroll$) by Table and Count}
\begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 15}{c}{} \\ 

\multicolumn{ 1}{c}{Table and $EmpTotal$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Payroll} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Intervals Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
\multicolumn{15}{c}{\textbf{Private}} \\ 
\input{\MyPathtv/tables/payroll_table_a.tex}
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Total Payroll is defined only over total employment. It is calculated by summing the earnings for the reference quarter for total employment.  See the table on total employment for the relevent counts. Statistics are computed across all state-year-quarters within a table. The ``Private" category of establishments includes private only private establishments. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for beginning of quarter employment, please see their respective equations in the accompanying text:  Total payroll \ref{eq:w1pub}, Total Variation \ref{eq:tvw1}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.  
 (a) Undefined value.
\end{tablenotes}
\label{tab:payrollpriv}
\end{threeparttable}
}%
\end{table}
\end{landscape}



==> tables/payroll_table_total.tex <==
\begin{landscape}
\begin{table}[htbp]
\resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \caption{Summary of Total Variability of All Total Payroll ($Payroll$) by Table and Count}
\begin{tabular}{lrrrrrrrrrrrrrr} \toprule 

\multicolumn{ 15}{c}{} \\ 

\multicolumn{ 1}{c}{Table and $EmpTotal$} & \multicolumn{ 1}{c}{Proportion} & \multicolumn{ 1}{c}{Number} & \multicolumn{ 1}{c}{Median} &  & \multicolumn{ 1}{c}{Median Total} & \multicolumn{ 1}{c}{Median Rubin Missingness} &  & \multicolumn{ 3}{c}{Quantiles of Coefficient} &  & \multicolumn{ 3}{c}{Median Approximate 90\%} \\ 
\multicolumn{ 1}{c}{count range} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{of Cells} & \multicolumn{ 1}{c}{Payroll} &  & \multicolumn{ 1}{c}{Variation} & \multicolumn{ 1}{c}{Rate (Percent)} &  & \multicolumn{ 3}{c}{of Variation} &  & \multicolumn{ 3}{c}{Confidence Intervals Margin of Error} \\ \cmidrule{9-11} \cmidrule{13-15}
\multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{ 1}{c}{} & \multicolumn{ 1}{c}{} &  & \multicolumn{1}{c}{5th} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{95th} &  & \multicolumn{1}{c}{Median df} & \multicolumn{1}{c}{Count} & \multicolumn{1}{c}{Percent} \\ \midrule
\multicolumn{15}{c}{\textbf{All (Private plus State and Local)}} \\ 
\input{\MyPathtv/tables/payroll_table_b.tex}
\bottomrule
\end{tabular}
\footnotesize
\begin{tablenotes}
\item {\it Notes}: Total Payroll is defined only over total employment. It is calculated by summing the earnings for the reference quarter for total employment.  See the table on total employment for the relevent counts. Statistics are computed across all state-year-quarters within a table. The ``All" category of establishments includes private as well as state, and local government but excludes federal employment. All tables include all valid QWI age groups with the exception of any table including education, in which case only jobs with workers age 25 and older are included. For statistic definitions for beginning of quarter employment, please see their respective equations in the accompanying text:  Total payroll \ref{eq:w1pub}, Total Variation \ref{eq:tvw1}, Missingness Ratio \ref{eq:mr}, Coefficient of Variation \ref{eq:cvc}.  
 (a) Undefined value.
\end{tablenotes}
\label{tab:payroll}
\end{threeparttable}
}%
\end{table}
\end{landscape}


